How Reliable is the Crowdsourced Knowledge of Security Implementation?

Stack Overflow (SO) is the most popular online Q&A site for developers to share their expertise in solving programming issues. Given multiple answers to certain questions, developers may take the accepted answer, the answer from a person with high reputation, or the one frequently suggested. However, researchers recently observed exploitable security vulnerabilities in popular SO answers. This observation inspires us to explore the following questions: How much can we trust the security implementation suggestions on SO? If suggested answers are vulnerable, can developers rely on the community's dynamics to infer the vulnerability and identify a secure counterpart? To answer these highly important questions, we conducted a study on SO posts by contrasting secure and insecure advices with the community-given content evaluation. We investigated whether SO incentive mechanism is effective in improving security properties of distributed code examples. Moreover, we also traced duplicated answers to assess whether the community behavior facilitates propagation of secure and insecure code suggestions. We compiled 953 different groups of similar security-related code examples and labeled their security, identifying 785 secure answer posts and 644 insecure ones. Compared with secure suggestions, insecure ones had higher view counts (36,508 vs. 18,713), received a higher score (14 vs. 5), and had significantly more duplicates (3.8 vs. 3.0) on average. 34% of the posts provided by highly reputable so-called trusted users were insecure. Our findings show that there are lots of insecure snippets on SO, while the community-given feedback does not allow differentiating secure from insecure choices. Moreover, the reputation mechanism fails in indicating trustworthy users with respect to security questions, ultimately leaving other users wandering around alone in a software security minefield.

==> data_old.tex <==
%%%%%%% begin: results generated by analysis scripts%%%%%
\newcommand\CCFinderGroups{2,657}
\newcommand\RelevantGroups{953}
\newcommand\IrrelevantGroups{1,704}
\newcommand\SecureGroups{585}
\newcommand\InsecureGroups{332}
\newcommand\MixedGroups{36}
\newcommand\RelevantInstances{3,121}
\newcommand\SecureInstances{1,784}
\newcommand\InsecureInstances{1,337}
\newcommand\IrrelevantInstances{5,569}
\newcommand\AllInstances{8,690}
\newcommand\SecureAnswers{781}
\newcommand\InsecureAnswers{648}
\newcommand\RelevantAnswers{1,429}
\newcommand\IrrelevantAnswers{2,133}
\newcommand\AllAnswers{3,562}
\newcommand\RelevantAnswersSSL{505}
\newcommand\SecureAnswersSSL{149}
\newcommand\InsecureAnswersSSL{356}
\newcommand\SecureAnswersRandom{14}
\newcommand\InsecureAnswersRandom{15}
\newcommand\SumCategoryAnswers{1,506}
\newcommand\AverViewsSecureAnswers{18,810}
\newcommand\AverViewsInsecureAnswers{36,280}
\newcommand\AverScoreSecureAnswers{5}
\newcommand\AverScoreInsecureAnswers{14}
\newcommand\AverCommentsSecureAnswers{2}
\newcommand\AverCommentsInsecureAnswers{3}
\newcommand\AverReputationSecureAnswers{18,637}
\newcommand\AverReputationInsecureAnswers{14,723}
\newcommand\AverFavoritesSecureAnswers{8}
\newcommand\AverFavoritesInsecureAnswers{15}
\newcommand\CoveredUsers{1,135}
\newcommand\SecureUsers{606}
\newcommand\InsecureUsers{558}
\newcommand\HighestReputation{990,402}
\newcommand\LowestReputation{1}
\newcommand\RelevantAnswersByTrustedUsers{208}
\newcommand\SecureAnswersByTrustedUsers{135}
\newcommand\InsecureAnswersByTrustedUsers{73}
\newcommand\AcceptedSecureAnswers{294}
\newcommand\AcceptedInsecureAnswers{242}
\newcommand\AcceptedRelevantAnswers{536}
\newcommand\HighReputationInsecureAnswers{27}
\newcommand\HighReputationRelevantAnswers{72}
\newcommand\UsersFirstFiveK{72}
\newcommand\AnswerReusageUsers{109}
\newcommand\SecureReusageUsers{67}
\newcommand\InsecureReusageUsers{48}
\newcommand\BothReusageUsers{6}
\newcommand\SecureGroupsOfReusedAnswers{112}
\newcommand\InsecureGroupsOfReusedAnswers{91}
\newcommand\MixedGroupsOfReusedAnswers{5}
\newcommand\RelevantGroupsOfReusedAnswers{208}
%%%%%%% end: results generated by analysis scripts  %%%%%%

%%%%%% please manually input the following results from the analysis script%%%

\newcommand\SecureGroupMeanSize{3.0}
\newcommand\InsecureGroupMeanSize{3.9}
\newcommand\GroupSizePValue{2.9e-5}
\newcommand\GroupSizeCliff{0.14}

\newcommand\ReusedPairsForDiffQ{46}
\newcommand\SecureSamplePairs{56}
\newcommand\MixedSamplePairs{2}
\newcommand\InsecureSamplePairs{45}


==> icse-2019-final-reviews.tex <==
----------------------- REVIEW 1 ---------------------
PAPER: 293
TITLE: How Reliable is the Crowdsourced Knowledge of Security Implementation?
AUTHORS: Mengsu Chen, Felix Fischer, Na Meng, Xiaoyin Wang and Jens Grossklags


----------- Summary -----------
This paper studies security related code snippets on StackOverflow to determine their level of security and how reliable they are. The sample of snippets studied is collected both through question tags related to security and also through snippets that match a predefined set of cryptography/security APIs as determined by Baker. Authors of the paper manually labeled the extracted snippets as secure/insecure/irrelevant based on a set of criteria described by previous work. The paper then presents various social statistics about the snippets such as their distribution w.r.t the reputation of the poster, score, views etc. as well as how the number of secure/insecure posts evolved over time. The conclusions of the paper suggest that there is no reliable measure to identify secure code snippets on StackOverflow and that better tool support or a different incentive system may be needed.

----------- Detailed Evaluation -----------
This paper was very easy to follow and was clear in almost all its aspects. As I was reading the introduction, I thought what could possibly be the new contribution as previous work has already established that a lot of posts on SO are insecure. However, the paper pleasantly surprised me that it had a more detailed investigation of the relation between the snippet security and different aspects on SO. I think the paper investigates different aspects than previous work, and it is interesting to see all the relationships within the context of different types of code snippets (encryption, TLS connections etc.). 

I have some questions and comments for improvement:

* One of the conclusions is that they authors did not find users who purposely propagated vulnerable code to mislead people. While I also doubt that this was anyone's intention, I don't think the authors have any evidence to claim that, as you cannot know people's intentions and someone who is purposely posting misleading code would not say so on their profile. Perhaps this sentence can be removed or toned down.

* I have worked with Baker before and I know that there are a lot of cases where (1) there are multiple matches for given element and (2) when there are no matches for the element. Both these cases depend on the oracle you use so my question is did you populate your own oracle with the set of APIs you chose? Did the oracle only contain these APIs such that case 1 is reduced a bit? Did you actually face any of case 1? What about case 2? What did you do in each case. I guess a reasonable condition can be that you only consider things where at least one element has an exact match (i.e., only 1) to one of your considered APIs. I would like to see that explicitly stated in the methodology and perhaps the innaccuracies or corner cases of Baker also discussed in the threats to validity, because such inaccuracies could have caused you to miss snippets too.

* I was a bit confused as to what exactly was examined in the 2,657 clone groups. Somewhere, it said that it is impossible to manually examine 25,855 snippets which is why clone groups were created. However, in section C, it also says "we manually examined each snippet in the 2,657 clone groups" so that was kind of confusing. I'm assuming one representitive snippet of each group was selected? If so, how selected? If you do not examine each snippet, how do you provide the labels? 

* Can you perhaps elaborate more on the 64% of clone groups that were still irrelevant. Perhaps name a few reasons so others can know what the limitations of your identifying techniques are?

* "Therefore, we label the post as "insecure" if any of the contained snippets is insecure; otherwise, if at least one snippet is secure, the post is labeled "secure"". These two conditions are not mutually exclusive. Is this intentional or a wording issue? Are you intentionally giving insecurity the priority?

* In III-D, I believe the numbers 19,662 and 23,224 appear for the first time there and it is a bit confusing where they came from. Perhaps mention them in section A when you talk about Baker?

* In Fig 4., where did the mixed category go?

* Thanks for Table IV!

* In terms of the reasons identified at the end of section IV before finding 8, wouldn't such cases be down voted by the community or at least receive negative comments? (where they don't directly answer the question or just advertise their library)

----------- Strengths and Weaknesses -----------
+ very well-written
+ determining security of crowd-source knowledge is both important and interesting
+ new contributions despite of similar previous work
+ authors aware of most of the threats to their work and explicitly discuss them
- investigation of clone groups can be elaborated
- JavaBaker may need to be discussed in some more details and in threats

----------- Author Question 1 -----------
Can you elaborate if every code snippet was examined or if only representative ones from the clone groups were labelled?

----------- Author Question 2 -----------
Can you describe what your criteria for Baker matching a code snippet to a security API was?


----------------------- REVIEW 2 ---------------------
PAPER: 293
TITLE: How Reliable is the Crowdsourced Knowledge of Security Implementation?
AUTHORS: Mengsu Chen, Felix Fischer, Na Meng, Xiaoyin Wang and Jens Grossklags


----------- Summary -----------
This paper describes an empirical study aimed to analyze the phenomenon of sharing insecure code through StackOverflow (SO) posts. The authors focused on vulnerabilities introduced by the misuse of Java security libraries. Some of the aspects the study investigates are related to a) how widespread are SO answers including insecure code; b) when are such answers more widespread; c) what is the popularity (upvotes, views, accepted answers) of answers including insecure code; d) what is the reputation of individuals posting secure and insecure source code. The study also investigated the reason why SO users may propagate very similar code across answers. The paper concludes providing recommendations to software developers, SO developers and designers of crowdsourcing platforms.

----------- Detailed Evaluation -----------
Significance
The paper illustrates a set of interesting findings. I found particularly intriguing that a big percentage of the code posted in the SO answers may be vulnerable. Also metrics to measure popularity of answers such as (number of upvotes, acceptance, views, reputation of the answerer) are not informative for indicating how secure the code contained in the answer is.  

However, this is not the first study in this direction. As the authors also acknowledge, Fischer et al. [5] conducted an empirical study to assess whether answer posts on SO include vulnerable code. Similarly to this paper, Fisher et al. also highlight that answers including insecure code did not receive lower scores compared to answers posting secure code. Although in this paper the authors also investigate other popularity metrics (answer acceptance, views, reputation of the answerer, repetitiveness), the findings are very similar.
In this paper the authors also investigate group of code snippets that are very similar but represent insecure and secure solutions and found out that differences between those solutions are in the parameters passed to security APIs.
Moreover although in paper [5] the authors focused on Android posts, the definition of security-relevant SO posts is the same, because both approaches are aimed to analyse misuses of the security libraries in the same categories.

The recommendations provided to software developers are rather general and could be applicable independently from the fact that insecure code is shared through SO. It would be useful to any software developer to have some sort of vulnerability scanner for source code that allows to pinpoint vulnerable code. In this space there is  already a lot of literature on attack surface detection. Some of the existing methods use static analysis to detect vulnerabilities caused by code cloning [1-4] and rule-based methods adopting analyst-generated rules to detect vulnerabilities [5,6]. Therefore I am wondering how the results of existing previous work can be exploited in such direction?

[1] Kim, Seulbae, Seunghoon Woo, Heejo Lee, and Hakjoo Oh. "VUDDY: a scalable approach for vulnerable code clone discovery." In Security and Privacy (SP), 2017 IEEE Symposium on, pp. 595-614. IEEE, 2017.
[2] Jang, Jiyong, Abeer Agrawal, and David Brumley. "ReDeBug: finding unpatched code clones in entire os distributions." In Security and Privacy (SP), 2012 IEEE Symposium on, pp. 48-62. IEEE, 2012.
[3] Pham, Nam H., Tung Thanh Nguyen, Hoan Anh Nguyen, and Tien N. Nguyen. "Detection of recurring software vulnerabilities." In Proceedings of the IEEE/ACM international conference on Automated software engineering, pp. 447-456. ACM, 2010.
[4] Li, Zhen, Deqing Zou, Shouhuai Xu, Hai Jin, Hanchao Qi, and Jie Hu. "VulPecker: an automated vulnerability detection system based on code similarity analysis." In Proceedings of the 32nd Annual Conference on Computer Security Applications, pp. 201-213. ACM, 2016.
[5] FlawFinder https://dwheeler.com/flawfinder/
[6] Checkmarx https://www.checkmarx.com/

In Finding 7 the authors suggests that highly similar code snippets performing distinct parameter passing to the same security API indicate the presence of a vulnerability. However, if a tool recognising such a vulnerability was going to be implemented I am wondering what would be its false positive rate and how generalizable this statement is.

Moreover it is difficult to get information about vulnerabilities patches; vendors hardly release this information and in many cases they do fix vulnerabilities silently. Therefore, designing new approaches that compare identified insecure implementations with secure counterparts may be difficult. This poses concerns in relation to the realizability of the suggestions provided in Sections VI.a and VI.b

Soundness
The empirical study was conducted rigorously.
However, there are aspects that are not completely clear.
The notion of “security-related” code refers to misuse of Java security libraries, such as those used to establish SSL/TLS connections, to support symmetric and asymmetric encryption, hashing and so on. The authors should justify why they have decided to consider that as a definition of security-related vulnerabilities. The chosen definition of security-related code partially accounts for the different ways in which security vulnerabilities can be introduced. Vulnerabilities can also be introduced when, for example, if branches do not have corresponding else branch or when the level of loop nesting increases, or when certain types of third-party libraries are adopted. Therefore I am wondering how generalisable are the results obtained by the authors. 

One of the other reasons that may support Finding 3 (on average insecure posts received a higher score) is the fact that posts containing insecure code are less recent and may have accumulated more positive scores than recent ones.

It is also unclear the suggestion of indicating the reputation score of the answerer "in related areas or for the specific tag" (Last suggestion in Section VI.b). How would such area- or tag- specific reputation score be computed?

Verifiability
The authors provide a lot of data to support the findings of the empirical study. For reproducibility purposes the information related to the extracted code snippets and their classification could have been shared publicly. 

Presentation
The paper is well structured and clear in all its parts.

The description of category “Symmetric” category indicates that cryptographic keys and initialisation vectors are insecure if they are “zeroed, statically assigned or directly derived from text”. However, Table I does not reflect what is indicated in the description.

To derive finding 2 the authors performed the Mann-Whitney U test and calculated the effect size. However, it is a bit unclear what does the effect size represent. Does it indicate that the difference (in terms of years) between more recent and less recent posts is big?

----------- Strengths and Weaknesses -----------
Strengths
* The paper describes interesting findings highlighting lack of correlation between posting vulnerable code on Stack Overflow and the popularity of the answer and the reputation of the answerer
* The empirical study was performed rigorously; 25855 code snippets have been labelled as secure or insecure depending on a set of rules described in previous work
* The paper is very clear and easy to read

Weaknesses
* The results of the paper do not appear very novel
* It is hard to understand how the recommendations highlighted at the end of the paper could be applied in practice.
* The scope of the paper refers to misuse of Java security libraries and does not consider other vulnerabilities that may be related to the code complexity or the use of external libraries.

----------- Author Question 1 -----------
Can you provide concrete suggestions about how the recommendations given to software developers, SO developers and crowdsourcing platforms designers can be applied in practice?

----------- Author Question 2 -----------
Why did you consider misuse of Java security libraries as your definition of security-related code? How generalizable is your approach to other Java source code vulnerabilities?


----------------------- REVIEW 3 ---------------------
PAPER: 293
TITLE: How Reliable is the Crowdsourced Knowledge of Security Implementation?
AUTHORS: Mengsu Chen, Felix Fischer, Na Meng, Xiaoyin Wang and Jens Grossklags


----------- Summary -----------
This paper addresses two main research questions: How much security implementation suggestions from Stack Overflow (SO) can be trusted? And, “if suggested answers are vulnerable, can developers rely on the community’s dynamics to infer the vulnerability and identify a secure counterpart?” The answer in both cases is No, i.e., there is a lot of Insecure code on SO, and insecure code is not detected by the community. On the contrary, insecure code (answers) received more votes, comments, favorites, and views than secure code (answers).

----------- Detailed Evaluation -----------
This paper addresses 2 important research questions (significance). The methods used are sound and can likely be replicated (Soundness and Verifiability). Authors do recognize their limitations in a section of the paper (VII. THREATS TO VALIDITY). Finally, the paper is easy to read and is well-structured (Presentation).

This is a very nice paper.

----------- Strengths and Weaknesses -----------
Strengths
- paper is well-structured and organized. Easy to read and follow;

- the methodology is described in a good level of detail. The libraries explored are important ones (in my limited understanding about the topic);

- overall, it presents interesting results;

- the paper presents a section about Recommendation for different types of stakeholders. This was really nice.

- the paper does a proper literature review discussing major work in the area, and clearly comparing its own work with them;

Weaknesses 

see my two questions.

Minor:
- I suggest removing this from the introduction: “Counterintuitively, since insecurity has no negative impact on answers’ score and the observed insecure answers have higher scores on average, users may have more incentives for duplicating insecure posts than secure posts on SO. However, so far, we have not identified any user that purposely propagated vulnerable code to mislead people.” This is pure speculation and not backed by any data.

- I think you switched values: “93% of Asymmetric posts, 70% of Hash posts, and 54% of Symmetric posts” should be “93% of Symmetric posts, 70% of Hash posts, and 54% of Asymmetric posts”.

----------- Author Question 1 -----------
One answer is labeled insecure if that contains a snippet of code labelled insecure. This might exaggerate the number of insecure answers. For instance, what if, one presents a NOT-to do example (insecure) followed by a HOW-TO (secure) example? That would be labelled as insecure. How this approach can influence your results?

----------- Author Question 2 -----------
Author Question 2: Finding 1 focus on all answers for one question. But, I wonder whether one reader would look into ALL or even SEVERAL different answers to the question. Wouldn’t be easier to focus on the ACCEPTED answer? What would be the results for Finding 1 if only the, arguably most important, answer (the ACCEPTED one) were analyzed?


-------------------------  METAREVIEW  ------------------------
PAPER: 293
TITLE: How Reliable is the Crowdsourced Knowledge of Security Implementation?

The reviewers found the paper interesting, rigorous, clear, and replicable, and appreciated the clarifications in the author response. The decision is to accept. I recommend the authors incorporate all of their clarifications and address the reviewers editing comments in the final revisions.

==> icse2019-reviews.tex <==
----------------------- REVIEW 1 ---------------------
PAPER: 293
TITLE: How Reliable is the Crowdsourced Knowledge of Security Implementation?
AUTHORS: Mengsu Chen, Felix Fischer, Na Meng, Xiaoyin Wang and Jens Grossklags

Poster Paper: no

----------- Summary -----------
This paper studies security related code snippets on StackOverflow to determine their level of security and how reliable they are. The sample of snippets studied is collected both through question tags related to security and also through snippets that match a predefined set of cryptography/security APIs as determined by Baker. Authors of the paper manually labeled the extracted snippets as secure/insecure/irrelevant based on a set of criteria described by previous work. The paper then presents various social statistics about the snippets such as their distribution w.r.t the reputation of the poster, score, views etc. as well as how the number of secure/insecure posts evolved over time. The conclusions of the paper suggest that there is no reliable measure to identify secure code snippets on StackOverflow and that better tool support or a different incentive system may be needed.

----------- Detailed Evaluation -----------
This paper was very easy to follow and was clear in almost all its aspects. As I was reading the introduction, I thought what could possibly be the new contribution as previous work has already established that a lot of posts on SO are insecure. However, the paper pleasantly surprised me that it had a more detailed investigation of the relation between the snippet security and different aspects on SO. I think the paper investigates different aspects than previous work, and it is interesting to see all the relationships within the context of different types of code snippets (encryption, TLS connections etc.). 

I have some questions and comments for improvement:

* One of the conclusions is that they authors did not find users who purposely propagated vulnerable code to mislead people. While I also doubt that this was anyone's intention, I don't think the authors have any evidence to claim that, as you cannot know people's intentions and someone who is purposely posting misleading code would not say so on their profile. Perhaps this sentence can be removed or toned down.

* I have worked with Baker before and I know that there are a lot of cases where (1) there are multiple matches for given element and (2) when there are no matches for the element. Both these cases depend on the oracle you use so my question is did you populate your own oracle with the set of APIs you chose? Did the oracle only contain these APIs such that case 1 is reduced a bit? Did you actually face any of case 1? What about case 2? What did you do in each case. I guess a reasonable condition can be that you only consider things where at least one element has an exact match (i.e., only 1) to one of your considered APIs. I would like to see that explicitly stated in the methodology and perhaps the innaccuracies or corner cases of Baker also discussed in the threats to validity, because such inaccuracies could have caused you to miss snippets too.

* I was a bit confused as to what exactly was examined in the 2,657 clone groups. Somewhere, it said that it is impossible to manually examine 25,855 snippets which is why clone groups were created. However, in section C, it also says "we manually examined each snippet in the 2,657 clone groups" so that was kind of confusing. I'm assuming one representitive snippet of each group was selected? If so, how selected? If you do not examine each snippet, how do you provide the labels? 

* Can you perhaps elaborate more on the 64% of clone groups that were still irrelevant. Perhaps name a few reasons so others can know what the limitations of your identifying techniques are?

* "Therefore, we label the post as "insecure" if any of the contained snippets is insecure; otherwise, if at least one snippet is secure, the post is labeled "secure"". These two conditions are not mutually exclusive. Is this intentional or a wording issue? Are you intentionally giving insecurity the priority?

* In III-D, I believe the numbers 19,662 and 23,224 appear for the first time there and it is a bit confusing where they came from. Perhaps mention them in section A when you talk about Baker?

* In Fig 4., where did the mixed category go?

* Thanks for Table IV!

* In terms of the reasons identified at the end of section IV before finding 8, wouldn't such cases be down voted by the community or at least receive negative comments? (where they don't directly answer the question or just advertise their library)

----------- Strengths and Weaknesses -----------
+ very well-written
+ determining security of crowd-source knowledge is both important and interesting
+ new contributions despite of similar previous work
+ authors aware of most of the threats to their work and explicitly discuss them
- investigation of clone groups can be elaborated
- JavaBaker may need to be discussed in some more details and in threats

----------- Author Question 1 -----------
Can you elaborate if every code snippet was examined or if only representative ones from the clone groups were labelled?

----------- Author Question 2 -----------
Can you describe what your criteria for Baker matching a code snippet to a security API was?

----------------------- REVIEW 2 ---------------------
PAPER: 293
TITLE: How Reliable is the Crowdsourced Knowledge of Security Implementation?
AUTHORS: Mengsu Chen, Felix Fischer, Na Meng, Xiaoyin Wang and Jens Grossklags

Poster Paper: no

----------- Summary -----------
This paper describes an empirical study aimed to analyze the phenomenon of sharing insecure code through StackOverflow (SO) posts. The authors focused on vulnerabilities introduced by the misuse of Java security libraries. Some of the aspects the study investigates are related to a) how widespread are SO answers including insecure code; b) when are such answers more widespread; c) what is the popularity (upvotes, views, accepted answers) of answers including insecure code; d) what is the reputation of individuals posting secure and insecure source code. The study also investigated the reason why SO users may propagate very similar code across answers. The paper concludes providing recommendations to software developers, SO developers and designers of crowdsourcing platforms.

----------- Detailed Evaluation -----------
Significance
The paper illustrates a set of interesting findings. I found particularly intriguing that a big percentage of the code posted in the SO answers may be vulnerable. Also metrics to measure popularity of answers such as (number of upvotes, acceptance, views, reputation of the answerer) are not informative for indicating how secure the code contained in the answer is.  

However, this is not the first study in this direction. As the authors also acknowledge, Fischer et al. [5] conducted an empirical study to assess whether answer posts on SO include vulnerable code. Similarly to this paper, Fisher et al. also highlight that answers including insecure code did not receive lower scores compared to answers posting secure code. Although in this paper the authors also investigate other popularity metrics (answer acceptance, views, reputation of the answerer, repetitiveness), the findings are very similar.
In this paper the authors also investigate group of code snippets that are very similar but represent insecure and secure solutions and found out that differences between those solutions are in the parameters passed to security APIs.
Moreover although in paper [5] the authors focused on Android posts, the definition of security-relevant SO posts is the same, because both approaches are aimed to analyse misuses of the security libraries in the same categories.

The recommendations provided to software developers are rather general and could be applicable independently from the fact that insecure code is shared through SO. It would be useful to any software developer to have some sort of vulnerability scanner for source code that allows to pinpoint vulnerable code. In this space there is  already a lot of literature on attack surface detection. Some of the existing methods use static analysis to detect vulnerabilities caused by code cloning [1-4] and rule-based methods adopting analyst-generated rules to detect vulnerabilities [5,6]. Therefore I am wondering how the results of existing previous work can be exploited in such direction?

[1] Kim, Seulbae, Seunghoon Woo, Heejo Lee, and Hakjoo Oh. "VUDDY: a scalable approach for vulnerable code clone discovery." In Security and Privacy (SP), 2017 IEEE Symposium on, pp. 595-614. IEEE, 2017.
[2] Jang, Jiyong, Abeer Agrawal, and David Brumley. "ReDeBug: finding unpatched code clones in entire os distributions." In Security and Privacy (SP), 2012 IEEE Symposium on, pp. 48-62. IEEE, 2012.
[3] Pham, Nam H., Tung Thanh Nguyen, Hoan Anh Nguyen, and Tien N. Nguyen. "Detection of recurring software vulnerabilities." In Proceedings of the IEEE/ACM international conference on Automated software engineering, pp. 447-456. ACM, 2010.
[4] Li, Zhen, Deqing Zou, Shouhuai Xu, Hai Jin, Hanchao Qi, and Jie Hu. "VulPecker: an automated vulnerability detection system based on code similarity analysis." In Proceedings of the 32nd Annual Conference on Computer Security Applications, pp. 201-213. ACM, 2016.
[5] FlawFinder https://dwheeler.com/flawfinder/
[6] Checkmarx https://www.checkmarx.com/

In Finding 7 the authors suggests that highly similar code snippets performing distinct parameter passing to the same security API indicate the presence of a vulnerability. However, if a tool recognising such a vulnerability was going to be implemented I am wondering what would be its false positive rate and how generalizable this statement is.

Moreover it is difficult to get information about vulnerabilities patches; vendors hardly release this information and in many cases they do fix vulnerabilities silently. Therefore, designing new approaches that compare identified insecure implementations with secure counterparts may be difficult. This poses concerns in relation to the realizability of the suggestions provided in Sections VI.a and VI.b

Soundness
The empirical study was conducted rigorously.
However, there are aspects that are not completely clear.
The notion of “security-related” code refers to misuse of Java security libraries, such as those used to establish SSL/TLS connections, to support symmetric and asymmetric encryption, hashing and so on. The authors should justify why they have decided to consider that as a definition of security-related vulnerabilities. The chosen definition of security-related code partially accounts for the different ways in which security vulnerabilities can be introduced. Vulnerabilities can also be introduced when, for example, if branches do not have corresponding else branch or when the level of loop nesting increases, or when certain types of third-party libraries are adopted. Therefore I am wondering how generalisable are the results obtained by the authors. 

One of the other reasons that may support Finding 3 (on average insecure posts received a higher score) is the fact that posts containing insecure code are less recent and may have accumulated more positive scores than recent ones.

It is also unclear the suggestion of indicating the reputation score of the answerer "in related areas or for the specific tag" (Last suggestion in Section VI.b). How would such area- or tag- specific reputation score be computed?

Verifiability
The authors provide a lot of data to support the findings of the empirical study. For reproducibility purposes the information related to the extracted code snippets and their classification could have been shared publicly. 

Presentation
The paper is well structured and clear in all its parts.

The description of category “Symmetric” category indicates that cryptographic keys and initialisation vectors are insecure if they are “zeroed, statically assigned or directly derived from text”. However, Table I does not reflect what is indicated in the description.

To derive finding 2 the authors performed the Mann-Whitney U test and calculated the effect size. However, it is a bit unclear what does the effect size represent. Does it indicate that the difference (in terms of years) between more recent and less recent posts is big?

----------- Strengths and Weaknesses -----------
Strengths
* The paper describes interesting findings highlighting lack of correlation between posting vulnerable code on Stack Overflow and the popularity of the answer and the reputation of the answerer
* The empirical study was performed rigorously; 25855 code snippets have been labelled as secure or insecure depending on a set of rules described in previous work
* The paper is very clear and easy to read

Weaknesses
* The results of the paper do not appear very novel
* It is hard to understand how the recommendations highlighted at the end of the paper could be applied in practice.
* The scope of the paper refers to misuse of Java security libraries and does not consider other vulnerabilities that may be related to the code complexity or the use of external libraries.

----------- Author Question 1 -----------
Can you provide concrete suggestions about how the recommendations given to software developers, SO developers and crowdsourcing platforms designers can be applied in practice?

----------- Author Question 2 -----------
Why did you consider misuse of Java security libraries as your definition of security-related code? How generalizable is your approach to other Java source code vulnerabilities?

----------------------- REVIEW 3 ---------------------
PAPER: 293
TITLE: How Reliable is the Crowdsourced Knowledge of Security Implementation?
AUTHORS: Mengsu Chen, Felix Fischer, Na Meng, Xiaoyin Wang and Jens Grossklags

Poster Paper: no

----------- Summary -----------
This paper addresses two main research questions: How much security implementation suggestions from Stack Overflow (SO) can be trusted? And, “if suggested answers are vulnerable, can developers rely on the community’s dynamics to infer the vulnerability and identify a secure counterpart?” The answer in both cases is No, i.e., there is a lot of Insecure code on SO, and insecure code is not detected by the community. On the contrary, insecure code (answers) received more votes, comments, favorites, and views than secure code (answers).

----------- Detailed Evaluation -----------
This paper addresses 2 important research questions (significance). The methods used are sound and can likely be replicated (Soundness and Verifiability). Authors do recognize their limitations in a section of the paper (VII. THREATS TO VALIDITY). Finally, the paper is easy to read and is well-structured (Presentation).

This is a very nice paper.

----------- Strengths and Weaknesses -----------
Strengths
- paper is well-structured and organized. Easy to read and follow;

- the methodology is described in a good level of detail. The libraries explored are important ones (in my limited understanding about the topic);

- overall, it presents interesting results;

- the paper presents a section about Recommendation for different types of stakeholders. This was really nice.

- the paper does a proper literature review discussing major work in the area, and clearly comparing its own work with them;

Weaknesses 

see my two questions.

Minor:
- I suggest removing this from the introduction: “Counterintuitively, since insecurity has no negative impact on answers’ score and the observed insecure answers have higher scores on average, users may have more incentives for duplicating insecure posts than secure posts on SO. However, so far, we have not identified any user that purposely propagated vulnerable code to mislead people.” This is pure speculation and not backed by any data.

- I think you switched values: “93\% of Asymmetric posts, 70\% of Hash posts, and 54\% of Symmetric posts” should be “93\% of Symmetric posts, 70\% of Hash posts, and 54\% of Asymmetric posts”.

----------- Author Question 1 -----------
One answer is labeled insecure if that contains a snippet of code labelled insecure. This might exaggerate the number of insecure answers. For instance, what if, one presents a NOT-to do example (insecure) followed by a HOW-TO (secure) example? That would be labelled as insecure. How this approach can influence your results?

----------- Author Question 2 -----------
Author Question 2: Finding 1 focus on all answers for one question. But, I wonder whether one reader would look into ALL or even SEVERAL different answers to the question. Wouldn’t be easier to focus on the ACCEPTED answer? What would be the results for Finding 1 if only the, arguably most important, answer (the ACCEPTED one) were analyzed?

------------------------------------------------------

==> mengsu-icse-2019-4/abstract.tex <==
\begin{abstract}

Stack Overflow (\SO) %TODO: change StO to SO
is the most popular online 
Q\&A site for developers to share their expertise in solving programming issues. 
Given multiple answers to certain questions, developers 
may take the accepted answer, the answer from a person with high reputation, or the one frequently suggested. 
%the solution recommended most often. 
However, researchers recently observed that \SO contains exploitable security vulnerabilities in the suggested code of popular answers, which found their way into security-sensitive high-profile applications that millions of users install every day.
This observation inspires us to explore the following questions: How much can we trust the security implementation suggestions on \SO? If suggested answers are vulnerable, can developers rely on the community's dynamics to infer the vulnerability and identify a secure counterpart?

 %Prior research shows that SO is one of the most important information resources that developers rely on, although the website contains security vulnerabilities in the suggested code of accepted answers. 
%A natural question raised by these observations is: how much can we trust the recommended security implementation on SO? 

%We conducted a comprehensive study on \SO posts related to the usage of Java security libraries. 
To answer these highly important questions, we conducted a comprehensive study on security-related \SO posts by contrasting secure and insecure advice with the community-given content evaluation. Thereby, we investigated whether \so{}'s gamification approach on incentivizing users is effective in improving security properties of distributed code examples. Moreover, we traced the distribution of duplicated samples over given answers to test whether the community behavior facilitates or prevents propagation of secure and insecure code suggestions within \so{}.
%After detecting duplicated coding suggestions that either use JCE APIs securely or insecurely, we compare the two kinds of suggestions for their frequency, the community's responses to them, the degree of duplication, and potential reasons for duplication. 
%After identifying \RelevantGroups\ groups of code clones that use security APIs, 

We compiled \RelevantGroups\ different groups of similar security-related code examples
%we revealed 1784 secure code snippets and 1339 insecure snippets, which correspond to 781 secure answer posts and 650 insecure answer posts. 
%we mapped the clones to \SecureAnswers\ secure answer posts and \InsecureAnswers\ insecure answer posts.  
and labeled their security, identifying \SecureAnswers\ secure answer posts and \InsecureAnswers\ insecure answer posts.  
%Among these posts, there were considerably more insecure suggestions than secure ones on SSL usage (\InsecureAnswersSSL\ vs.~\SecureAnswersSSL).
Compared with secure suggestions, insecure ones had higher view counts (\AverViewsInsecureAnswers\ vs.~\AverViewsSecureAnswers),
received a higher score (\AverScoreInsecureAnswers\ vs.~\AverScoreSecureAnswers),
and had significantly more duplicates (\InsecureGroupMeanSize\ vs.~\SecureGroupMeanSize) on average. 34\% of the posts provided by highly reputable so-called \textit{trusted users} were insecure.  %TODO Na: give numbers
%\SO users provided many insecure answers to solve coding issues, without mentioning the resulting vulnerabilities. 
%Many insecure answers were suggested to solve coding issues, and the answerers did not mention the resulting vulnerabilities. 
% seemed to be unaware of the resulting vulnerabilities. 
%Secure suggestions have not obtained significantly more favorite counts or votes than insecure ones.  
%Interestingly, we also identified 48 users that repetitively posted the same insecure answers, although they appeared to be unaware of the vulnerabilities. 
%Our findings reveal the widespread existence of insecure suggestions on \SO, and the community's lack of expertise and incentives to discriminate between insecure and secure code. 
%Therefore, developers cannot fully rely on the crowd-sourced knowledge of security implementation provided by \so{}. 

Our findings show that based on the distribution of secure and insecure code on \so{}, users being laymen in security rely on additional advice and guidance.
However, the community-given feedback does not allow  differentiating secure from insecure choices. The reputation mechanism fails in indicating trustworthy users with respect to security questions, ultimately leaving other users wandering around alone in a software security minefield.
%blindly %TODO: weak claim->they cannot rely on the feedback system provided by SO 


%Since majority voting (MV) has been considered as the optimal decision rule for merging multiple answers into a single reliable one, our study focused on the duplicated (in)secure code examples using JCE APIs. 
%With secure and insecure code examples collected, 
%we compared their frequency, the community's responses to them, the degree of duplication, and potential reasons for duplication. 
\end{abstract}

\begin{IEEEkeywords}
Stack Overflow,
crowdsourced knowledge, 
social dynamics, 
security implementation
\end{IEEEkeywords}

==> mengsu-icse-2019-4/background.tex <==
\section{Background}
\label{sec:background}

To facilitate the discussion of \SO community activities around security implementations, we will first introduce \SO's crowdsourcing model, and then summarize the domain knowledge used to label secure and insecure code snippets. 

\begin{figure}
\includegraphics[width=8.5cm]{Figure_post.pdf}
\caption{A typical \SO discussion thread contains one question post and one or multiple answer posts~\cite{exemplarso}}
\label{fig:so}
\vspace{-1.5em}
\end{figure}
\subsection{Stack Overflow as a Crowdsourcing Platform}
Some observers believe that the success of \SO lies in its crowdsourcing model and the reputation system~\cite{so_crowd,so_crowdsourced_2010}. 
The four most common forms of participation are i) question asking, ii) question answering, iii) commenting, and iv) voting/scoring~\cite{so_crowd}. 
Figure~\ref{fig:so} presents an exemplar \SO discussion thread, which contains one question and one or many answers.  
When multiple answers are available, the asker decides which answer to \textbf{accept}, and marks it with ``\textcolor{green}{\cmark}''. 

%Experts are motivated to answer questions because they enjoy helping people or gain reputation for solving technical challenges~\cite{incentive_so}.
After a user posts a question, an answer, or a comment, other users can vote for or against the post. 
Users gain \textbf{reputation} for each up-vote their posts receive. 
For instance, answers earn their authors 10 points per up-vote, questions earn 5, and comments earn 2~\cite{what-reputation}. 
All users initially have only one reputation point. 
As users gain more reputation, they are granted more administrative privileges to help maintain \SO posts~\cite{so-priviledges}. For instance, a user with 15 points can vote up posts. A user with 125 points can vote down posts. Users with at least 20K points are considered ``\textbf{trusted users}'', and can edit or delete other people's posts. %In our research, we consider such trusted users as \textbf{people with high reputation}. 

The \textbf{score} of a question or answer post is decided by the up-votes and down-votes the post received. 
Users can \textbf{favorite} a question post if they want to bookmark the question and keep track of any update on the discussion thread. 
% bookmark the question, and later check back for an update on the question or related responses. 
Each question contains one or many \textbf{tags}, which are words or phrases to describe topics of the question.
Each post has a \textbf{timestamp} to show
when it was created. 
Each discussion thread has a \textbf{view count} to indicate how many times the thread has been viewed.% and a \textbf{timestamp} to indicate when the question was asked. 

\subsection{Categorization of Java Security Implementations}
Based on state-of-the-art security knowledge, researchers defined five categories of security issues relevant to library misuses~\cite{fischer:2017}.
Table~\ref{tab:rules} shows their criteria, which we use in this project to decide whether a code snippet is insecure or not. 
% SSL/TLS, symmetric cryptography, asymmetric cryptography, one way hash functions, and (secure) random number generation. 

\begin{table}
\caption{Criteria used to decide code's security property}
\label{tab:rules}
\vspace{-0.5em}
\scriptsize
\begin{tabular}{C{1.5cm}|C{2.3cm}|C{3.7cm}}
\toprule
\textbf{Category} & \textbf{Parameter} & \textbf{Insecure} \\ 
\toprule
\multirow{5}{*}{\textbf{SSL/TLS}} & HostnameVerifier & allow all hosts
\\ \cline{2-3}
& Trust Manager & trust all %, bad pinning, validity only
\\ \cline{2-3}
& Version & $<$TLSv1.1 
%{SSLContext sslContext = SSLContext.getInstance("TLS");}
\\ \cline{2-3}
& {Cipher Suite} & RC4, 3DES, AES-CBC
MD5, MD2\\ \cline{2-3}
& {OnReceivedSSLError} & proceed
\\ \toprule
& {Cipher/Mode} & RC2, RC4, DES, 3DES, AES/ECB, Blowfish\\ \cline{2-3}
\textbf{\symmetric} & {Key} & static, bad derivation\\ \cline{2-3}
%\textbf{Cryptography}
& Initialization Vector (IV) & zeroed, static, bad derivation\\ \cline{2-3} 
& Password Based Encryption (PBE) & $<$1k iterations, $<$64-bit salt, static salt  
\\ \toprule
\textbf{Asymmetric} 
%& Padding & PKCS8, OAEPWithSHA-256 AndMGF1Padding\\ \cline{2-3}
%\textbf{Cryptography} 
& Key &RSA $<$ 2,048 bit, ECC $<$ 224 bit 
%& {KeyPairGenerator kpg = KeyPairGenerator.getInstance("RSA");}
%{kpg.initialize(1024);}
 \\ \toprule
%\textbf{One Way} 
& PBKDF & $<$SHA224, MD2, MD5 \\ \cline{2-3}
\textbf{\hash}& Digital Signature & SHA1, MD2, MD5\\ \cline{2-3} 
%\textbf{Functions}
& Credentials & SHA1, MD2, MD5\\ \toprule
%\textbf{(Secure) Random} 
& Type & Random \\ \cline{2-3}
\textbf{\random }& Seeding & setSeed$\rightarrow$nextBytes, setSeed with static values %& {byte[] keyStart = "encryption key".getBytes();} {SecureRandom sr = SecureRandom.getInstance("SHA1PRNG");} {sr.setSeed(keyStart); // set seed with static value}
\\ 
\bottomrule
\end{tabular}
\vspace{-1.5em}
\end{table}

\paragraph*{\textbf{SSL/TLS}}
There are five key points concerning how to \emph{securely} establish SSL/TLS connections. First, developers should use an implementation of the \codefont{HostnameVerifier} interface
%to check whether a given certificate's common name matches the server's hostname. 
to verify servers' hostnames instead of allowing all hosts~\cite{Fahl:2012}. 
Second, when implementing a custom \codefont{TrustManager}, developers should validate certificates instead of blindly trusting all certificates. 
Third, when ``TLS'' is passed as a parameter to  \codefont{SSLContext.getInstance(...);}, developers should explicitly specify the version number to be at least 1.1, because TLS' lower versions are insecure~\cite{Sheffer2015}.
Fourth, the usage of insecure cipher suites should be avoided. Fifth, 
when overriding \codefont{onReceivedSslError()}, developers should handle instead of skipping any certificate validation error. 
Listing~\ref{lst:ssl} shows a vulnerable snippet that allows all hosts, trusts all certificates, and uses TLS v1.0.

\lstset{
%numbers=left, 
basicstyle=\scriptsize,
%numberstyle=\small, 
%numbersep=2pt, 
breaklines=true,
escapeinside={(*}{*)},
frame = tb}
\begin{lstlisting}[caption=An example to demonstrate 
three scenarios of insecurely using SSL/TLS APIs~\cite{trust-all-allow-all}, label={lst:ssl}]
(*\bfseries // Create a trust manager that does not validate certificate chains (trust all)*)
private TrustManager[] trustAllCerts = new TrustManager[] {
  new X509TrustManager() {
    public java.security.cert.X509Certificate[] getAcceptedIssuers() {return null;}
    public void checkClientTrusted(...) {}
    public void checkServerTrusted(...) {}    }};    
public ServiceConnectionSE(String url) throws IOException {
  try {
    (*\bfseries // Use the default TLSv1.0 protocol *)
    SSLContext sc = SSLContext.getInstance("TLS");
    (*\bfseries // Install the trust-all trust manager*)
    sc.init(null, trustAllCerts, new java.security.SecureRandom()); ... } ...
  connection = (HttpsURLConnection) new URL(url).openConnection();
  (*\bfseries // Use AllowAllHostnameVerifier that allows all hosts *)
  ((HttpsURLConnection) connection).setHostnameVerifier(new AllowAllHostnameVerifier());    }  
\end{lstlisting}

\paragraph*{\textbf{\symmetric}} 
There are ciphers and modes of operations known to be insecure. Cryptographic keys and initialization vectors (IV) are insecure if they are statically assigned, zeroed, or directly derived from text. Password Based Encryption (PBE) is insecure if the iteration number is less than 1,000, the salt's size is smaller than 64 bits, or a static salt is in use. Listing~\ref{lst:symmetric} presents a vulnerable code example that insecurely declares a cipher, a key, and an IV. 

\begin{lstlisting}[caption=An example to present 
several 
insecure usage scenarios of symmetric cryptography~\cite{keyiv}, label=lst:symmetric]
(*\bfseries // Declare a key parameter with a static value*)
private static byte[] key = "12345678".getBytes();
(*\bfseries // Declare an IV parameter with a static value*)
private static byte[] iv = "12345678".getBytes();
public static String encrypt(String in) {
  String cypert = in;
  try {
    IvParameterSpec ivSpec = new IvParameterSpec(iv);
    (*\bfseries // Create a secret key with the DES cipher*)
    SecretKeySpec k = new SecretKeySpec(key, "DES");
    (*\bfseries // Declare a DES cipher*)
    Cipher c = Cipher.getInstance("DES/CBC/PKCS7Padding");
    c.init(Cipher.ENCRYPT_MODE, k, ivSpec);
    ... }    }
\end{lstlisting}

\paragraph*{\textbf{\asymmetric}}
Suppose that a code snippet uses either RSA or ECC APIs to generate keys. 
When the specified key lengths for RSA and ECC are separately shorter than 2,048 bits and 224 bits, we consider the API usage to be insecure. Listing~\ref{lst:asymmetric} shows a vulnerable code example. 

\begin{lstlisting}[caption=An example that insecurely uses RSA by specifying the key size to be 1024~\cite{asymmetric}, label=lst:asymmetric]
KeyPairGenerator kpg = KeyPairGenerator.getInstance("RSA");
kpg.initialize(1024);
KeyPair kp = kpg.generateKeyPair();
RSAPublicKey pub = (RSAPublicKey) kp.getPublic();
RSAPrivateKey priv = (RSAPrivateKey) kp.getPrivate();
\end{lstlisting}

\paragraph*{\textbf{\hash}}
In the context of password-based key derivation, digital signatures, and authentication/authorization, developers may explicitly invoke broken hash functions. Listing~\ref{lst:hash} shows an example using MD5.

\begin{lstlisting}[caption=Insecurely creating a message digest with MD5~\cite{md5}, label=lst:hash]
final MessageDigest md = MessageDigest.getInstance("md5");
(*\bfseries // It is also insecure to hardcode the plaintext password*)
final byte[] digestOfPassword = md.digest("HG58YZ3CR9".getBytes("utf-8"));
\end{lstlisting}

\paragraph*{\textbf{\random}}
To make the generated random numbers unpredictable and secure, developers should use \codefont{SecureRandom} instead of \codefont{Random}. When using \codefont{SecureRandom}, developers can either (1) call \codefont{nextBytes()} only, or (2) call \codefont{nextBytes()} first and \codefont{setSeed()} next. Developers should not call \codefont{setSeed()} with static values. Listing~\ref{lst:sr} presents an example using \codefont{SecureRandom} insecurely. 

\begin{lstlisting}[caption=Using \codefont{SecureRandom} with a static seed~\cite{sr}, label=lst:sr]
byte[] keyStart = "encryption key".getBytes();
SecureRandom sr = SecureRandom.getInstance("SHA1PRNG");
sr.setSeed(keyStart);
\end{lstlisting}

==> mengsu-icse-2019-4/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We aimed to assess the reliability of the crowdsourced knowledge on security implementation. Our analysis of 1,429 answer posts on \SO revealed 3 insights. 
\begin{enumerate}
\item In general secure and insecure advices more or less balance each other (55\% secure and 45\% insecure). Users without security knowledge may heavily rely on the community to provide helpful feedback in order to identify secure advice. Unfortunately, we found the community's feedback to be almost useless. 
For certain cryptographic API usage scenarios, the situation is even worse: insecure coding suggestions about SSL/TLS dominate the available options. This is particularly alarming as SSL/TLS is one of the most common use cases in production systems according to prior work~\cite{fischer:2017}.
%\item Although fewer than secure coding suggestions, there are still many insecure suggestions on \SO. For certain security categories and some years, the insecure answers dominate the website, without including any information to explicitly warn about the vulnerabilities. 

\item The reputation mechanism and voting system popularly used in crowdsourcing platforms turn out to be powerless to remove or discourage insecure suggestions. Insecure answers were suggested by people with high reputation and widely accepted as easy fixes for programming errors. On average, insecure answers received more votes, comments, favorites, and views than secure answers.
As a countermeasure, security evaluation can be included in the voting and reputation system to establish missing incentives for providing secure and correcting insecure content.
%Worsely, a crowdsourcing platform can even promote insecure answers when the majority of contributors do not know or care about the security issues.

\item %The design of crowdsourced platforms needs more work. %Currently at \SO, users with 15 reputation points can vote up posts, but only users with 125 points can vote down posts. Such design discourages security experts to down-vote insecure answers if the experts do not have enough reputation.
When users are motivated to earn reputation by answering more questions, the platform encourages contributors to provide duplicated, less useful, or insecure coding suggestions. Therefore, with respect to security, \so{}'s gamification approach counteracts its original purpose as it promotes distribution of secure and insecure code. Although we did not identify any malicious user that misuses \SO to propagate insecure code, we do not see any mechanism designed to prevent such malicious behaviors, either.

\end{enumerate}

When developers refer to crowdsourced knowledge as one of the most important information resources, 
it is crucially important to enhance the quality control of crowdsourcing platforms. This calls for a strong collaboration between developers, security experts, tool builders, educators, and  platform providers. By educating developers to contribute high-quality security-related information, and integrating vulnerability and duplication detection tools into platforms, we can improve software quality via crowdsourcing. Our future work is focused on building the needed tool support. 

==> mengsu-icse-2019-4/data.tex <==

%%%%%%% results begin %%%%%
\newcommand\CCFinderGroups{2,657}
\newcommand\RelevantGroups{953}
\newcommand\IrrelevantGroups{1,704}
\newcommand\SecureGroups{587}
\newcommand\InsecureGroups{326}
\newcommand\MixedGroups{40}
\newcommand\RelevantInstances{3,121}
\newcommand\SecureInstances{1,802}
\newcommand\InsecureInstances{1,319}
\newcommand\IrrelevantInstances{5,569}
\newcommand\AllInstances{8,690}
\newcommand\TotalSnippet{25,855}
\newcommand\SecureAnswers{785}
\newcommand\InsecureAnswers{644}
\newcommand\AllAnswers{3,562}
\newcommand\TotalAnswers{23,224}
\newcommand\ExcludedAnswers{19,662}
\newcommand\RelevantAnswers{1,429}
\newcommand\IrrelevantAnswers{2,133}
\newcommand\RelevantAnswersSSL{505}
\newcommand\SecureAnswersSSL{150}
\newcommand\InsecureAnswersSSL{355}
\newcommand\SecureAnswersRandom{15}
\newcommand\InsecureAnswersRandom{14}
\newcommand\SumCategoryAnswers{1,506}
\newcommand\AverViewsSecureAnswers{18,713}
\newcommand\AverViewsInsecureAnswers{36,508}
\newcommand\AverScoreSecureAnswers{5}
\newcommand\AverScoreInsecureAnswers{14}
\newcommand\AverCommentsSecureAnswers{2}
\newcommand\AverCommentsInsecureAnswers{3}
\newcommand\AverReputationSecureAnswers{18,654}
\newcommand\AverReputationInsecureAnswers{14,678}
\newcommand\AverFavoritesSecureAnswers{8}
\newcommand\AverFavoritesInsecureAnswers{15}
\newcommand\CoveredUsers{1,135}
\newcommand\SecureUsers{610}
\newcommand\InsecureUsers{554}
\newcommand\HighestReputation{990,402}
\newcommand\LowestReputation{1}
\newcommand\RelevantAnswersByTrustedUsers{208}
\newcommand\SecureAnswersByTrustedUsers{137}
\newcommand\InsecureAnswersByTrustedUsers{71}
\newcommand\AcceptedSecureAnswers{297}
\newcommand\AcceptedInsecureAnswers{239}
\newcommand\AcceptedRelevantAnswers{536}
\newcommand\HighReputationInsecureAnswers{26}
\newcommand\HighReputationRelevantAnswers{72}
\newcommand\UsersFirstFiveK{72}
\newcommand\AnswerReusageUsers{109}
\newcommand\SecureReusageUsers{66}
\newcommand\InsecureReusageUsers{49}
\newcommand\BothReusageUsers{6}
\newcommand\SecureGroupsOfReusedAnswers{111}
\newcommand\InsecureGroupsOfReusedAnswers{90}
\newcommand\MixedGroupsOfReusedAnswers{6}
\newcommand\RelevantGroupsOfReusedAnswers{207}
%%%%%%% results end  %%%%%%

%%%%%% please manually input the following results from the analysis script%%%
\newcommand\SecureGroupMeanSize{3.0}
\newcommand\InsecureGroupMeanSize{3.8}
\newcommand\GroupSizePValue{1.3e-4}
\newcommand\GroupSizeCliff{0.13}

\newcommand\ReusedPairsForDiffQ{46}
\newcommand\SecureSamplePairs{56}
\newcommand\MixedSamplePairs{2}
\newcommand\InsecureSamplePairs{45}



==> mengsu-icse-2019-4/evaluation.tex <==
\section{Major Findings}
\label{sec:evaluation}
%Our results are shown in Section~\ref{sec:rq1}-Section~\ref{sec:rq4}.
In this section, we present our results and discuss the main findings regarding our stated research questions.

\input{rq1}

\input{rq2}

\input{rq3}

\input{rq4}













==> mengsu-icse-2019-4/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Since its launch in 2008, Stack Overflow (\SO) has served as the infrastructure for developers to discuss programming-related questions online, and provided the community with crowdsourced knowledge~\cite{so_crowdsourced,so_crowdsourced_2010}. Prior work shows that \SO is one of the most important information resources that developers rely on~\cite{mamykina_design_2011,Acar:2016}. Meanwhile, researchers also revealed that some highly upvoted,
or even accepted answers on \SO contained insecure code% which might have been incorporated into developers' software products
~\cite{fischer:2017,Meng2018:icse}. 
More alarmingly, Fischer \emph{et al.}~found that insecure code snippets from \SO were copied and pasted into 196,403 Android applications available on Google Play~\cite{fischer:2017}. 
Several high-profile applications containing particular instances of these insecure snippets were successfully attacked, and user credentials, credit card numbers and other private data were stolen as a result~\cite{Fahl:2012}.
%The exploitation of vulnerable code in many applications allows hackers to steal user credentials, credit card numbers, and other private data~\cite{Fahl:2012}.

%TODO: Further, it has been shown that many instances of this severely vulnerable code have been reused in security-sensitive high-profile applications millions of users install from Google Play everyday~\cite{fischer:2017}. Based on these vulnerabilities many applications were succesfully attacked, stealing user credentials, credit card numbers and other private data~\cite{fahl:2011}.
These observations made us curious about SO's reliability regarding suggestions for security implementations. 
%the popularity of insecure code snippets on SO. 
Taking a pessimistic view, such insecure suggestions can be expected to be prevalent on the Q\&A site, and consistent corrective feedback by the programming community may be amiss. Consequently, novice developers may learn about incorrect crowdsourced knowledge from such Q\&A sites, propagate the misleading information to their software products or other developers, and eventually make our software systems vulnerable to known security attacks.% TODO: this sentence is way to long

%For this paper, we conducted \emph{a comprehensive in-depth investigation into the popularity of both secure and insecure coding suggestions on \SO, and the community activities around those two kinds of suggestions}. To ensure a fair comparison between secure and insecure suggestions, we focused on the discussion threads related to Java security. % TODO: new sentence
%We used JavaBaker~\cite{Subramanian:2014} to mine for answer posts that contained any code using security libraries, and extracted 25,855 such code snippets.
%%Because we are not aware of any tool that accurately decides whether a code fragment is secure or not, %TODO: imprecise, there are many tools
%We reused the security domain expertise summarized by prior work~\cite{fischer:2017} to manually label whether a given code snippet is secure or not. 
%However, different from prior work~\cite{fischer:2017} that studied the application of insecure \SO answers to production code, 
%our work focuses on the SO suggestions themselves. %TODO: new sentence
%More specifically, we studied coding suggestions' popularity, social dynamics, and duplication. We also inquired 
%%acquire a big picture 
%how developers %TODO: developers?
%may be misled by insecure answers on \SO. 

%whether a code snippet uses APIs securely or insecurely.
%Previous work has identified particular cryptographic use cases that are prevalent in discussions on \so{}, as well as in production code. Due to their prevalence, similar and duplicated code snippets have been detected in many different questions and answers. Moreover, their view count was significantly higher than less prevalent topics, leading to a higher copy-and-paste rate in real-world applications. However, the majority of the provided code examples was highly insecure.
%One example is the problem of applying transport layer security (TLS) in Android. Almost 15\% of applications available on Google Play were effected by insecure code stemming from these discussions. The reused code example which was responsible for hundreds of thousands of applications being vulnerable had the highest view count from all inspected insecure code snippets and several comments that warned against applying it~\cite{fischer:2017}.  

Therefore, within this paper, we conducted \emph{a comprehensive in-depth investigation of the popularity of both secure and insecure coding suggestions on \SO, and the community activities around them}. To ensure a fair comparison between secure and insecure suggestions, we focused on the discussion threads related to Java security. % TODO: new sentence
We used Baker~\cite{Subramanian:2014} to mine for answer posts that contained any code using security libraries, and extracted 25,855 such code snippets.
%%Because we are not aware of any tool that accurately decides whether a code fragment is secure or not, %TODO: imprecise, there are many tools
We reused the security domain expertise summarized by prior work~\cite{fischer:2017} to manually label whether a given code snippet is secure or not. 
However, different from prior work~\cite{fischer:2017} that studied the application of insecure \SO answers to production code, 
our work focuses on the SO suggestions themselves. %TODO: new sentence
More specifically, we studied coding suggestions' popularity, social dynamics, and duplication. We also inquired 
%%acquire a big picture 
how developers %TODO: developers?
may be misled by insecure answers on \SO. 
%Therefore, within this paper we want to identify hot-topics in security to investigate the following research questions (RQs)

To identify prevalent topics on \so{}, we used CCFinder~\cite{Kamiya2002} to detect code clones (\emph{i.e.}, duplicated code) in the data extracted by Baker. These clones are clustered within clone groups. \RelevantGroups\ clone groups were observed to use security library APIs and implement functionalities like SSL/TLS, symmetric and asymmetric encryption, \emph{etc.} 
Moreover, we found that code examples within clone groups are more likely to be viewed than non-duplicated code snippets on \so{}. This further motivates our sampling method as we can expect clones to have a higher impact on users and production code. %according to~\cite{fischer:2017}. 
Among the \RelevantGroups\ clone groups, 
%groups of clones detected in the complete set of security-related code snippets, %TODO: what are clone groups?
there were \SecureGroups\ groups of duplicated secure code,
\InsecureGroups\ groups of similar insecure code, and \MixedGroups\ groups with a mixture of secure and insecure code snippets. % TODO: what are these three groups?
These clone groups covered \SecureInstances\ secure code snippets and \InsecureInstances\ insecure ones. 
By mapping cloned code to their container posts, 
we contrasted insecure suggestions with secure ones in terms of their popularity, users' feedback, degree of duplication, and causes for duplication. 
%the extent and causes of duplication between secure and insecure answers. %TODO: this needs some more explanation
%With our thorough manual analysis of coding suggestions and statistical hypothesis testing to compare secure and insecure answers, 

We explored the following Research Questions (RQs):

\begin{itemize}
\setlength\itemsep{0.5em}
%TODO: 1) already investigated in prior work -> no novelty
\item \textbf{RQ1:} \emph{How prevalent are insecure coding suggestions on \SO?} 
Prior work witnessed the existence of vulnerable code on \SO, and indicates that such code can mislead developers and compromise the quality of their software products~\cite{Acar:2016,fischer:2017,Meng2018:icse}. To understand the number and growth of secure and insecure options that developers have to choose from, we (1) compared the occurrence counts of insecure and secure answers, and (2) observed the distributions of both kinds of answers across a 10-year time frame (2008-2017).
%As a viable heuristic, if secure answers are usually posted later than insecure ones, a developer without much security expertise could rely on answers' timestamps to identify secure answers. 

\item \textbf{RQ2:} \emph{Do the community dynamics or \SO's reputation mechanism help developers choose secure answers over insecure ones?}
Reputation mechanisms and voting were introduced to crowdsourcing platforms to (1) incentivize contributors to provide high-quality solutions, and (2) facilitate question askers to identify responders with high expertise~\cite{Jurczyk:2007,Xie2015,Katmada2016}.
We conducted statistical testing to compare secure and insecure answers in terms of votes, answerers' reputations, \emph{etc.} %Hypothetically, if secure answers received more votes or the providers of secure suggestions usually have higher reputations, a user could trust such community dynamics to select secure answers over insecure ones. %TODO shorten


%Contrasting secure and insecure answers, we inquired whether answerers' reputation and other users' behaviors triggered by the reputation system reflect different patterns?%TODO: I dont understand this sentence

\item \textbf{RQ3:} \emph{Do secure coding suggestions have more  duplicates than insecure ones?}
%\textbf{Majority voting} has been considered as the most commonly used consensus-based method to mitigate erroneous information on crowd-sourcing platforms~\cite{Nitzan1982,mv,Tao2018}. %TODO: This sentence has nothing to do with the rest of this item!? You investigate duplicate counts not voting right? Or both?
When certain answers are repetitively suggested, it is %quite
likely that developers will encounter such answers more often. Moreover, if these answers are provided by different users, the phenomenon might facilitate users' trust in the answers' correctness.
Therefore, we compared the degree of repetitiveness for insecure and secure answers.
%Ideally, if there are always more duplicates of secure answers than insecure ones, developers could rely on duplicated \SO answers to identify secure solutions. 
%trust duplicated answers to guarantee the security property of suggestions. 
%TODO: Wether insecure code samples have many duplicates is rather boring. Interesting are the reasons why? E.g. does duplication have a positive impact on reputation? If you report that the gamification approach of SO facilitates distribution of insecure over secure code, you have a very important finding. Becuase users are rewarded for insecure code, there are no incentives to provide secure code instead.

%\item \textbf{RQ4:} \emph{Did developers intentionally suggest duplicated insecure answers?}
%Theoretically, if malicious users want to mislead developers to build vulnerable software, it is feasible for them to misuse SO by repetitively posting insecure code. We located the users that provided duplicated insecure answers, and examined their user profiles. 
\item \textbf{RQ4:} \emph{Why did users suggest duplicated secure or insecure answers on \SO?}
We were curious about why certain code was repetitively suggested, and we explored this facet of community behavior by examining the duplicated answers posted by the same or different users.
%The answer to this question will not only shed light on new approaches of detecting duplicated \so posts, but also help prevent potential  \emph{misinformation attacks}, \emph{i.e.}, the misleading information (\emph{e.g.}, insecure code) intentionally propagated on \SO by malicious users. 
% Namely, if malicious users want to mislead developers to build vulnerable software, they can misuse \SO by repetitively posting insecure code. 
% to explore the reasons.%TODO: Actually this is the most interesting and difficult research question
%We located user that provided duplicated answers, and studied why th

\end{itemize}

In our study, we made four major observations:
\begin{enumerate}
\setlength\itemsep{0.5em}
\item \emph{As with secure answers, insecure answers are prevalent on \SO across the entire studied time frame.} 
The inspected \RelevantInstances\ snippets from different clone groups correspond to \SecureAnswers\ secure posts and \InsecureAnswers\ insecure ones.  %with some of the posts containing multiple snippets. 
%More alarmingly, 
Among the \RelevantAnswersSSL\ SSL/TLS-related posts, \InsecureAnswersSSL\ posts (70\%) suggest insecure solutions, which makes SSL/TLS-related answers the most unreliable ones on \so{}.
At least 41\% of the security-related answers posted every year are insecure, which shows that security knowledge on \so{} in general is not significantly improving over time. %means that developers cannot rely on answers' timestamps to identify secure solutions.%, as both secure and insecure answers span over the years. 

\item \emph{The community dynamics and SO's reputation mechanisms are not reliable indicators for secure and insecure answers.} 
Compared with secure posts, insecure ones obtained higher \emph{scores}, more \emph{comments}, more \emph{favorites}, and more \emph{views}. 
Although the providers of secure answers received significantly higher \emph{reputation} scores, the effect size is negligible ($<$0.147). 
%(1) there are significant differences in terms of the comment count, answerer's reputation, and view count, but the effect size is negligible ($\le$0.147); (2) there is no significant difference for vote count and favorite count. 
\AcceptedInsecureAnswers\ of the \AcceptedRelevantAnswers\ examined \emph{accepted answers} (45\%) are insecure. 
\HighReputationInsecureAnswers\ out of the \HighReputationRelevantAnswers\ posts (36\%) suggested by ``trusted users'' (with $\ge$20K reputation scores~\cite{so-priviledges}) are insecure.
These observations imply that reputation and voting on \so{} are not reliable to help users distinguish between secure and insecure answers. %indicating that this reputation signal is unreliable when it comes to security. 
%Among the \todo{X} posts that received high votes ($\ge$Y), \todo{Y} posts are insecure. 
%TODO: I dont get anything from this! I dont understand it and I certainly dont see this as a "major observation". Please explain...

\item 
\emph{The degree of duplication among insecure answers is significantly higher than that of secure ones.} 
On average, 
there are more clones in an insecure group than a secure one (\InsecureGroupMeanSize\ vs.~\SecureGroupMeanSize). It means that users may have to deal with a large supply of insecure examples for certain questions, before obtaining secure solutions. 
%answers for particular questions, 
%which makes it even harder for users to pick the secure solutions. 
%which makes it even more likely to pick insecure solutions.
%developers cannot trust duplication to reveal secure answers. 
%On average, each insecure clone group has 4 snippets, while a secure group has 3 snippets. 
%Most clone groups contain only two snippets, 
%We also found \MixedGroups\ mixed clone groups where each group has both secure and insecure code.%, and the parameters sent to certain APIs decide whether a snippet is secure or not. 
% This finding will help researchers build security analysis tools. %TODO: Way to short in explanation! Reviewers wont understand it, I dont understand it.
% Each group contains both secure and insecure code that differs in terms of the parameters sent to security APIs. 
% each of which contains both secure and insecure code. 
%The biggest secure group contains 65 snippets, which generate release key hashes for any Android app interacting with Facebook. 
%The biggest insecure group has 32 clone instances, which establish SSL connections in a simple but vulnerable way. 

\item \emph{Users seem to post duplicated answers, while ignoring security as a key property.} 
Duplicated answers were provided due to duplicated questions or users' intent to answer more questions by reusing code examples.
This behavior is incentivized by the reputation system on \so{}. The more answers are posted by a user and up-ranked by the community, the higher reputation the user gains.
%Counterintuitively, since insecurity has no negative impact on answers' score and the observed insecure answers have higher scores on average, 
%users may have more incentives for duplicating insecure posts than secure posts on \so{}.
%Although \InsecureReusageUsers\ users reused insecure answers, 
%However, so far, we have not identified any user that 
%we did not identify any user that 
%purposely propagated vulnerable code to mislead people. 
%Among the \AnswerReusageUsers\ users that posted duplicated answers, \InsecureReusageUsers\ users reused insecure answers, \SecureReusageUsers\ users repetitively posted secure ones, and \BothReusageUsers\ users reused both secure and insecure answers. 
%In addition to the insecure answers, the \InsecureReusageUsers\ users also posted many other answers in different domains. 
%There are \todo{X} users who repetitively posted answers even though the answers are not quite relevant to the questions. 

%TODO: Generally, in my oppinon RQs and "major findings" are weakly descreibed and presented and need revision. I didnt really get what you want to find out and what you did find out.

\end{enumerate}
Our source code and data set are available at \url{https://github.com/mileschen360/Higgs}. 

==> mengsu-icse-2019-4/method.tex <==
\vspace{-0.5em}
\section{Methodology}
\label{sec:method}
%\vspace{-0.5em}

To collect secure and insecure answer posts, 
we first extracted code snippets from \SO that used any security API (Section~\ref{sec:extract}).
Next, we sampled the extracted code corpus by detecting duplicated code (Section~\ref{sec:clone}).
Finally, we manually labeled sampled code as secure, insecure, or irrelevant, and mapped the code to related posts (Section~\ref{sec:label}). 
Additionally, 
%to verify whether our clone-based sampling method included prevalent answer posts, 
we compared the view counts of the sampled posts vs.~unselected posts to check samples' prevalence
(Section~\ref{sec:cdf}). 


%Finally, we mapped the identified secure and insecure code to their related posts, and extracted additional information for hypothesis testing (Section~\ref{sec:testing}). 

\subsection{Code Extraction}
\label{sec:extract}
To identify coding suggestions, this step extracts security-related answer posts by analyzing (1) tags of question posts, and (2) the code snippets' API usage of answer posts.
After downloading the Stack Overflow data as XML files~\cite{datadump},  
%To facilitate data query and analysis, 
we used a tool stackexchange-dump-to-postgres~\cite{xmltotable} to convert the XML files to Postgres database tables. 
Each row in the database table ``Posts'' corresponds to one post. 
A post's body text may use the HTML tag pair 
\codefont{<code>} and \codefont{</code>} to enclose source code, so we leveraged this tag pair to extract code. 
Since there were over 40 million posts under processing, and one post could contain multiple code snippets, 
\emph{it is very challenging to efficiently identify security implementations from a huge amount of noisy code data.} 
Thus, we built two heuristic filters to quickly skip irrelevant posts and snippets. 

\begin{table}[!h]
\caption{Tags used to locate relevant \SO discussion threads}
\label{tab:tags}
\vspace{-0.5em}
\begin{tabular}{C{2cm}| p{6cm}}
\toprule
\textbf{Category} & \textbf{Tags}\\
\toprule
\textbf{Java platforms}
& android, applet, eclipse, java, java1.4, java-7, java-ee, javamail, jax-ws, jdbc, jndi, jni, ...
\\ \hline 
\textbf{Third-party tools/libraries} & axis2, bouncycastle, gssapi, httpclient, java-metro-framework, openssh, openssl, spring-security, ...\\ \hline
\textbf{Security} & aes, authentication, certificate, cryptography, des, encoding, jce, jks, jsse, key, random, rsa, security, sha, sha512, single-sign-on, ssl, tls, X509certificate, ...\\ 
\bottomrule
\end{tabular}
\vspace{-1em}
\end{table}

\subsubsection{Filtering by question tags}
As tags are defined by askers to describe the topics of questions, we relied on tags to skip obviously irrelevant posts. To identify as many security coding suggestions as possible, 
we inspected the 64 cryptography-related posts mentioned in prior work~\cite{Meng2018:icse}, and identified 93 tags. 
If a question post contains any of these tags, we extracted code snippets from the corresponding answer posts.
As shown in Table~\ref{tab:tags}, these tags are either related to Java platforms, third-party security libraries or tools, or security concepts. 
%We found the tags by analyzing the 64 cryptography-related posts mentioned in prior work. 

\subsubsection{Filtering by security API usage}
Similar to prior work~\cite{fischer:2017}, we used Baker~\cite{Subramanian:2014} to decide whether a snippet calls any security API. 
This paper focuses on the following APIs: 
\begin{itemize}
\item Java platform security: org.jetf.jgss.*, android.security.*, com.sun.security.*, java.security.*, javax.crypto.*, javax.net.ssl.*, javax.security.*, javax.xml.crypto.*; 
\item Third-party security libraries: 
BouncyCastle~\cite{bc},
GNU Crypto~\cite{gnu-crypto},
jasypt~\cite{jasypt}, 
keyczar~\cite{keyczar}, 
scribejava~\cite{scribejava},
SpongyCastle~\cite{sc}.
\end{itemize}
%To decide whether a code snippet invokes any security API, a naive approach can compare the methods invoked by the snippet with all known security APIs; if any method's name matches, the snippet is security-related. However, such naive approaches do not work well. They can cause many false positives and wrongly identify irrelevant code, because such approaches cannot differentiate between the methods with identical names but declared by different classes.
%Thus, we chose to use Baker to better locate security-related code. 
After taking in a set of libraries and a code snippet, Baker (1) extracts all APIs of types, methods, and fields from the libraries, (2) extracts names of types, methods, and fields, used in the code snippet, and (3) iteratively deduces identifier mappings between the extracted information.
Intuitively, when multiple type APIs (\emph{e.g.}, \codefont{a.b.C} and \codefont{d.e.C}) can match a used type name \codefont{C}, Baker compares the invoked methods on \codefont{C} against the method APIs declared by each candidate type, and chooses the candidate that contains more matching methods. 

We included a code snippet if Baker finds at least one API (class or method) with an exact match. However, Baker's result set is not fully accurate and requires a number of post-processing steps to reduce false positives. These include a blacklist filter for standard Java types (e.g., String) and very popular methods (e.g., get()). Baker's oracle contains only the given security APIs, which helped reduce false positives when detecting secure code but did not help reduce false negatives.  

\subsection{Clone Detection}
\label{sec:clone}
With the filters described above, we identified \TotalSnippet\ code snippets (from \TotalAnswers\ posts) that are probably security-related. 
%are likely to implement security. 
%We are not aware of any automatic tool that always correctly labels code's security property.
%It is almost impossible to manually check all these snippets to identify secure and insecure code. %Felix \emph{et al.~} built a machine learning model to automatically decide whether a snippet is secure or insecure with 90\% accuracy~\cite{fischer:2017}. Since the classification result directly affects 
Since it is almost impossible to manually check all these snippets to identify secure and insecure code, we decided to (1) sample representative extracted code via clone detection, and then (2) manually label the samples. 
In addition to sampling, clone detection facilitates our research in two further ways. 
%We decided to sample the extracted code via clone detection for two reasons. 
First, by identifying duplicated code with CCFinder~\cite{Kamiya2002}, we could explore the degree of duplication among secure and insecure code. 
Second, through clustering code based on their similarity, we could efficiently read similar code fragments, and determine their security property in a consistent way. 
%With the default parameter setting in CCFinder, we identified 2,657 clone groups that contained 8,690 code snippets.
With the default parameter setting in CCFinder, we identified \CCFinderGroups\ clone groups that contained \AllInstances\ code snippets, with each group having at least two snippets. 
%We manually inspected these \AllInstances\ snippets. 

\subsection{Code Labeling}
\label{sec:label}
%To label code snippets, 
%We first studied prior work's rule definition 
%~\cite{fischer:2017} and dataset~\cite{felixdataset} to learn the criteria of code labeling. Then, 
We manually examined each of those \AllInstances\ snippets and labeled code based on the criteria mentioned in Section~\ref{sec:background}.
%in the \CCFinderGroups\ clone groups to label code based on th
If a snippet meets any criteria of insecure code shown in Table~\ref{tab:rules}, it is labeled as ``insecure''. If the snippet uses any security API but does not meet any criteria, it is labeled as ``secure''; otherwise, it is ``irrelevant''. 
Depending on the APIs involved, we also decided to which security category a relevant post belongs. 
When unsure about certain posts, we had discussions to %ensure correct labeling and 
achieve consensus. 
Finally, we randomly explored a subset of the labeled data to double check the correctness. 
%The second author is a software engineering expert with some security experience, and the third author is a security expert. 

\begin{table}
\caption{Code labeling results for \CCFinderGroups\ clone groups}
\scriptsize
\centering
\label{tab:label}
\begin{tabular}{c| rrrr|r}
\toprule
 & \textbf{Secure} & \textbf{Insecure} & \textbf{Mixed} & \textbf{Irrelevant} & \textbf{Total}\\
\toprule
\textbf{\# of clone groups} &\SecureGroups\ & \InsecureGroups\ & \MixedGroups\ & \IrrelevantGroups\ & \CCFinderGroups\ \\ 
\textbf{\# of snippets} &\SecureInstances\ & \InsecureInstances\ & 0 &  \IrrelevantInstances\ & \AllInstances\ \\
\textbf{\# of answer posts} &\SecureAnswers\ & \InsecureAnswers\ & 0 & \IrrelevantAnswers\ & \AllAnswers\ \\ 
\bottomrule
\end{tabular}
\vspace{-0.5em}
\end{table}


Table~\ref{tab:label} presents our labeling results for the inspected \CCFinderGroups\ clone groups. After checking individual code snippets, we identified \SecureGroups\ secure groups, \InsecureGroups\ insecure groups, \MixedGroups\ mixed groups, and \IrrelevantGroups\ irrelevant groups. In particular, a mixed group has both secure snippets and insecure ones, which are similar to each other. Although two filters were used (see Section~\ref{sec:extract}), 64\% of the clone groups from refined data were still irrelevant to security,
which evidences the difficulty of precisely identifying security implementation with Baker.

%The clone groups correspond to \SecureInstances\ secure snippets, \InsecureInstances\ insecure snippets, and \IrrelevantInstances\ irrelevant ones. 
%When mapping these snippets to their owner answer posts, we identified \SecureAnswers\ secure posts, \InsecureAnswers\ insecure posts, and \IrrelevantAnswers\ irrelevant ones. 
%Particularly, 
%if multiple snippets correspond to the same answer post, as long as one of the snippets is insecure, we label the post as ``insecure''; otherwise, if at least one snippet is secure, we label the post as ``secure''. If a post does not contain any secure or insecure snippet, it is labeled as ``irrelevant''.  
The clone groups cover \SecureInstances\ secure snippets, \InsecureInstances\ insecure ones, and \IrrelevantInstances\ irrelevant ones. 
%When mapping these snippets to their owner answer posts, we identified \SecureAnswers\ secure answers, \InsecureAnswers\ insecure ones, and \IrrelevantAnswers\ irrelevant ones. One answer can have multiple snippets of different clone groups. Therefore, we label the post as ``insecure'' if any of the contained snippets is insecure; otherwise, if at least one snippet is secure, the post is labeled as ``secure''. 
When mapping these snippets to the answer posts (which contain them), we identified \SecureAnswers\ secure answers, \InsecureAnswers\ insecure ones, and \IrrelevantAnswers\ irrelevant ones. One answer can have multiple snippets of different clone groups. Therefore, 
we consider a post ``insecure'' if it contains any labeled insecure code. A post was labeled ``secure'' if it has no insecure snippet but at least one secure snippet. 
%A post was labeled ``irrelevant'' if it does not have any (in)secure snippet.
%we label the post as ``insecure'' if any of the contained snippets is insecure; otherwise, if at least one snippet is secure, the post is labeled as ``secure''. 
If a post does not contain any (in)secure snippet, it is labeled as ``irrelevant''. 

\subsection{Verifying the Prevalence of Sampled Posts}
\label{sec:cdf}

To check whether our clone-based approach actually included representative SO posts, we separately computed the cumulative distribution functions   (CDF)~\cite{Gentle:2009} of view count for 
the included \AllAnswers\ posts (as mentioned in Table~\ref{tab:label}), the excluded \ExcludedAnswers\ posts, %and all 23,224 posts that are related to the candidate security implementations reported by Baker.
and the complete set of 23,224 posts identified by Baker.
%The CDFs are plotted in 
%Fig.~\ref{fig:cdf}, where logarithmic scales are used for the horizontal axis because answers' view counts vary a lot. 
As shown in Fig.~\ref{fig:cdf}, the ``\textit{included}'' curve is beneath the ``\textit{all}'' and ``\textit{excluded}'' curves. This shows that the highly viewed answers take up a higher percentage in our sample set than the excluded answers. 
%This observation also indicates that it is meaningful to sample answers with clone detection, because this sampling method can retrieve more highly viewed or prevalent answers than random sampling. 
%because the highly viewed answers are more likely to be included  


\begin{figure}
\vspace{-0.5em}
\centering
\includegraphics[width=8cm]{CDF.pdf}
\vspace{-1.5em}
\caption{CDFs of view count among the included answers, excluded ones, and all answers related to Baker's output}
\label{fig:cdf}
\vspace{-1em}
\end{figure}

==> mengsu-icse-2019-4/related.tex <==
\section{Related Work}
\label{sec:related}

%This section describes 
%The related work is on security API misuses, developer studies, empirical studies on \SO, and clone detection for \SO. 

\subsection{Security API Misuses}

Prior studies showed that API misuses caused security vulnerabilities~\cite{LongSoftwareVulnerabilities2005,
Fahl:2012,Georgiev:2012,Egele:2013,Lazar:2014,veracode,Yang2016,fischer:2017}. 
For instance, 
Lazar et al.~analyzed 369 published cryptographic vulnerabilities in the CVE database, and found that 83\% of them were caused by API misuses
%the misuse of cryptographic libraries
~\cite{Lazar:2014}. 
%Veracode reported that 39\% of all applications used broken or risky cryptographic algorithms~\cite{veracode}. 
%Fahl \emph{et al.}~\cite{Fahl:2012} and Georgiev \emph{et al.}~\cite{Georgiev:2012} exploited developers' misuse of SSL/TLS and successfully fulfilled the man-in-the-middle (MITM) attack. 
Egele \emph{et al.}~built a static checker for six well-defined Android cryptographic API usage rules (e.g., ``Do not use ECB mode for encryption''). 
They analyzed 11,748 Android applications for any rule violation~\cite{Egele:2013}, and found 88\% of the applications violating at least one checked rule.
Instead of checking for insecure code in CVE or software products, we focused on \SO. 
Because the insecure coding suggestions on \SO can be read and reused by many  developers, they have a  profound impact on software quality.  

The research by Fischer \emph{et al.}~\cite{fischer:2017} is closely related to our work.
In their work, secure and insecure snippets from SO were used to search for code clones in Android apps. Our research is different in three aspects. First, it 
investigates the evolution and distribution of secure and insecure coding suggestions within the SO ecosystem itself.
Second, while [5] compares average score and view counts for secure and insecure snippets, they merely do this for snippets whose exact copies have migrated into apps but not for our much broader set of snippets on SO. Therefore, the dataset of [5] is not representative to evaluate the impact of severity, community's awareness, and popularity of unreliable SO suggestions on secure coding. 
Third, we conducted not only statistical testing on a comprehensive dataset to quantitatively contrast score, view count, comment count, reputation, and favorite count, but also case studies to qualitatively analyze the differences. We further explored the missing link between gamification and security advice quality on crowdsourcing platforms. 

%In their work, Android-related code snippets are extracted from \SO. The authors manually labeled a subset of the data as ``secure'' or ``insecure'', and used the data to train a classifier that automatically labels the remaining extracted data. With the labeled data, the authors searched for insecure code in Android apps via clone detection. Our research is different in two aspects. First, our research scope is different. We aimed to analyze the popularity, surrounding  social dynamics, and duplication of insecure code on \SO. 
%Second, our (in)security labeling is more reliable. As it is always challenging to determine whether a given snippet is secure or not, we chose to conduct manual analysis instead of using machine learning to accurately identify insecure code. 

\subsection{Developer Studies}
Researchers conducted interviews or surveys to understand  developers' security coding practices~\cite{xie_why_2011,balebako_improving_2014,Nadi:2016,Acar:2016}. 
For example, Nadi \emph{et al.} surveyed 48 developers and revealed that developers found it difficult to use cryptographic algorithms correctly~\cite{Nadi:2016}.
Xie \emph{et al.} interviewed 15 developers, and found that (1) most developers had reasonable knowledge about software security, but (2) they did not consider security assurance as their own  responsibility~\cite{xie_why_2011}.  
%that people other than themselves should be responsible to address security issues 
%Balebako and Cranor interviewed 19 and surveyed 228 developers about their privacy and security behaviors~\cite{balebako_improving_2014}. 
%Researchers observed developers' bad privacy practices, and identified several causes for that, such as (1) hard-to-read privacy policies, and (2) treating privacy as a secondary task. 
% found that developers had bad privacy practices, because (1) the privacy policies of third-party tools are hard to read; (2) writing privacy policies for their own apps is considered useless; or (3) privacy is considered a secondary task. 
Acar \emph{et al.} surveyed 295 developers and conducted a lab user study with 54 students and professional Android developers~\cite{Acar:2016}. 
They observed that most developers used search engines and \SO to address security issues. 
%; and (2) participants using \SO are more likely to produce functionally correct but insecure code than participants that use other resources (\emph{e.g.}, textbooks). 
These studies inspired us to explore how much we can trust the crowdsourced knowledge of security coding on \SO. 

\subsection{Empirical Studies on Stack Overflow}

Researchers conducted various studies on \SO~\cite{mamykina_design_2011,Bosu2013,Barua2014,Yang2016,rahman,Meng2018:icse,zhang_are_2018}. Specifically,   
Zhang \emph{et al.}~studied the JDK API usage recommended by \SO, and observed that 31\% of the studied posts misused APIs~\cite{Meng2018:icse}. 
%Yang \emph{et al.}~\cite{Yang2016} and Rahman~\cite{rahman} separately extracted security-relevant high-frequency keywords from \SO questions (\emph{e.g.}, ``Password'').  
Meng \emph{et al.} manually inspected 503 \SO discussion threads related to Java security~\cite{Meng2018:icse}. They revealed various secure coding challenges (\emph{e.g.}, hard-to-configure third-party frameworks) and vulnerable coding suggestions (\emph{e.g.}, SSL/TLS misuses). 
Mamykina \emph{et al.}~revealed several reasons (\emph{e.g.}, high response rate) to explain why \so is one of the most visible venues for expert knowledge sharing~\cite{mamykina_design_2011}.
%analyzed \SO to understand why this platform quickly became one of the most visible venues for expert knowledge sharing 
%They found that 93\% of questions are answered, and most answer activities take place in the first hours. 
Vasilescu \emph{et al.}~studied the associations between \SO and GitHub, and found that GitHub committers usually ask fewer questions and provide more answers~\cite{Vasilescu2013}.
%by mapping \SO users to GitHub committers~\cite{Vasilescu2013}. They revealed that GitHub committers take the role of a ``teacher'' by asking fewer questions and providing more answers. 
Bosu \emph{et al.}~analyzed the dynamics of reputation building on SO, and found that answering as many questions as possible can help users quickly earn reputation~\cite{Bosu2013}. 

%They found that participating regularly and answering as many questions as possible can help users quickly earn reputation. 

%being prompt to answer questions helps users quickly increase reputation. 

In comparison, our paper quantitatively and qualitatively analyzed secure and insecure \SO suggestions in terms of (1) their popularity, (2) answerers' reputations, (3) the community's feedback to answers  (\emph{e.g.}, votes and comments), and (4) the degree and causes of duplicated answers.  
We are not aware of any prior work that analyzes \SO posts in these aspects.  

% that analyzes SO posts in such ways. 

\subsection{Duplication Detection Related to SO or Vulnerabilities}

Researchers used clone detection to identify duplication within \so or between \so and software products
%or copy-and-paste practices between \SO and software products
~\cite{Chen:2015,ahasanuzzaman_mining_2016,An2017,zhang_detecting_2017,yang_stack_2017}. 
Specifically, Ahasanuzzaman \emph{et al.}~detected duplicated \SO questions with machine learning~\cite{ahasanuzzaman_mining_2016}. 
%Zhang \emph{et al.}~detected duplicated posts via latent semantics and association rules~\cite{zhang_detecting_2017}.
An \emph{et al.} compared code between \SO and Android apps and observed unethical code reuse phenomena on \SO~\cite{An2017}. 
%Yang \emph{et al.} found 1.9M Python snippets in GitHub projects to be clones of code in \SO~\cite{yang_stack_2017}. Chen and Kim built a
%tool to (1) search for \SO questions that have code clones of a given snippet under debugging, and (2)
%suggest code based on the related answer posts~\cite{Chen:2015}. 
Other researchers used static analysis to detect vulnerabilities caused by code cloning~\cite{Pham:2010:DRS,Jang:2012:ReDeBug,Li:2016:VAV,Kim2017:VUDDY}. For instance, Kim et al.~generate a fingerprint for each Java method to efficiently search for clones of a given vulnerable snippet~\cite{Kim2017:VUDDY}. 
Different from prior work, we did not invent new clone detection techniques or compare code between \so and software projects. 
%duplication detection techniques, neither did we focus on the code mapping between \SO and software projects. 
We used clone detection to (1) sample crawled security-related code, and (2) explore why \SO users 
posted similar code to answer questions. 



==> mengsu-icse-2019-4/rq1.tex <==
\subsection{Popularity of Secure and Insecure Code Suggestions}
\label{sec:rq1}

\begin{figure}
\centering
\includegraphics[width=8cm]{Figure_distribution-category.pdf}
\vspace{-2em}
\caption{The distribution of posts among different categories}
\label{fig:category}
\vspace{-1em}
\end{figure}

Figure~\ref{fig:category} presents the distribution of \RelevantAnswers\ answer posts among the 5 security categories. 
Since some posts contain multiple snippets of different categories, the total number of plotted secure and insecure posts in Figure~\ref{fig:category} is \SumCategoryAnswers, slightly larger than \RelevantAnswers. 
Among the categories, \emph{SSL/TLS} contains the most posts (34\%), %Symmetric (short for ``symmetric cryptography'') has the second most posts (29\%),
while \emph{Random} has the fewest posts (2\%). 
Two reasons can explain such a distribution. 
First, developers frequently use or are more concerned about APIs of \emph{SSL/TLS}, \emph{Symmetric}, and \emph{Hash}. 
Second, the criteria we used to label code contain more diverse rules for the above-mentioned three categories, so we could identify more instances of such code. 

There are many more insecure snippets than secure ones in the \emph{SSL/TLS}  (\InsecureAnswersSSL\ vs.~\SecureAnswersSSL) category, indicating that 
%and slightly more \todo{this is no longer true} insecure snippets for \emph{Random}  (\InsecureAnswersRandom\ vs.~\SecureAnswersRandom). 
developers should be quite cautious when searching for such code.
Meanwhile, secure answers dominate the other categories, accounting for 94\% of 
\emph{Asymmetric} posts, 71\% of \emph{Hash} posts, 54\% of \emph{Symmetric} posts, and 52\% of \emph{Random} posts. 
However, notice that across these 4 categories, only 67\% of the posts are secure;  
%can be considered secure. However, it is important to keep in mind that across these three categories still only 67\% of the postings are labeled secure; 
that is, considerable room for error remains. 
% THIS DOES NOT SOUND LIKE CREDIBLE ADVICE TO ME: It indicates that developers should choose \SO suggestions on Asymmetric over Symmetric, if both kinds of suggestions fulfill the same tasks (\emph{e.g.}, encryption and decryption); this is because answers of the former category are more reliable. 

\begin{tcolorbox}
	\textbf{Finding 1:}
	\emph{\InsecureAnswers\ out of the \RelevantAnswers\ inspected answer posts (45\%) are insecure, meaning that insecure suggestions popularly exist on \SO. 
	Insecure answers dominate, in particular, the SSL/TLS category. }
\end{tcolorbox}

\begin{figure}
\includegraphics[width=8cm]{Figure_distribution-time.pdf}
\caption{The distribution of posts over during 2008-2017}
\label{fig:time}
\vspace{-1.5em}
\end{figure}
To explore the distribution of secure and insecure answers over time, we clustered answers based on their timestamps. 
As shown in Figure~\ref{fig:time}, both types of answers increased year-by-year from 2008 to 2014, and decreased in 2015-2017. This may be because \so reached its saturation for Java security-related discussions in 2014-2015.  
In 2008, 2009, and 2011, insecure answers were posted more often than secure ones, taking up 53\%-100\% of the sampled data of each year. 
For the other years, secure posts constitute the majority within the yearly sampled data set, accounting for 53\%-59\%. 

To further determine whether older posts are more likely to be insecure, we considered 
post IDs as logical timestamps. We applied a Mann-Whitney U test
(which does not require normally distributed data~\cite{Fay2010}), and calculated the Cliff's delta size (which measures the difference's magnitude~\cite{MACBETH2011}).  
The resulting $p$-value is 0.02, with Cliff's $\Delta$=0.07. It means that secure answers are significantly more recent than insecure ones, but the effect size is negligible. %REDUNDANT: Therefore, insecure answers are likely to be older than secure answers, although only a small subset of the examined data evidences such phenomenon. 

Two reasons can explain this finding. First, some vulnerabilities were recently revealed.  
Among the 17 insecure posts in 2008 and 2009, 6 answers use MD5, 6 answers trust all certificates, and 4 answers use TLS 1.0. 
However, these security functions were found
broken in 2011-2012~\cite{flame,Georgiev:2012,Fahl:2012,duong2011}, which made the answers obsolete and insecure.  
Second, some secure answers were posted to correct insecure suggestions. For instance, we found a question inquiring about fast and simple string encryption/decryption in Java~\cite{secure_after_insecure}. The accepted answer in 2011 suggested DES---an insecure symmetric-key algorithm. 
%In response to this insecure answer, 
Later, various comments pinpointed the vulnerability and a secure answer was provided in 2013.

Note that there can be a significant lag until the community adopts new  secure technologies, and phases out technologies known to be insecure. 
Although MD5's vulnerability was exploited by Flame malware in 2012~\cite{flame}, as shown in Fig.~\ref{fig:md5}, 
MD5 was still popularly suggested afterwards, obtaining a peak number of related answers in 2014. 


\begin{tcolorbox}
	\textbf{Finding 2:}
	\emph{Insecure posts led the sampled data in 2008-2011, while secure ones were dominant afterwards. 
	%At least 40\% of the security-related answers posted every year are insecure.
	Older security-related posts are less reliable, likely because recently revealed vulnerabilities outdated older suggestions. We found only few secure answers suggested to correct outdated, insecure ones.  
	}
\end{tcolorbox} 

\begin{figure}
    \centering
    \includegraphics[width=8cm]{n-hash-answers-over-time.pdf}
    \vspace{-1em}
    \caption{Distributions of MD5 and SHA256 related posts}
    \label{fig:md5}
    \vspace{-1.5em}
\end{figure}

==> mengsu-icse-2019-4/rq2.tex <==
\begin{table*}
\caption{Comparison between secure and insecure posts}
\label{tab:all}
\vspace{-0.5em}
\scriptsize
\centering
\begin{tabular}{C{1.5cm}|C{2cm} R{2cm}R{2cm}R{2cm}R{2cm}R{2cm} }
\toprule
& & \textbf{Score} & \textbf{Comment count} & \textbf{Reputation} & \textbf{Favorite count} & \textbf{View count}\\
\toprule
\multirow{4}{*}{\textbf{All}} & \textbf{Secure mean} 
& 5 & 2 & 18,654 & 8 & 18,713\\ \cline{2-7}
& \textbf{Insecure mean} 
& 14 & 3 & 14,678 & 15 & 36,580\\ \cline{2-7}
& \textbf{p-value} 
& 0.97 & 0.02& 0.02& 0.09& 1.5e-3\\ \cline{2-7}
& \textbf{Cliff's $\Delta$}
& - & 0.07 (negligible) & 0.07 (negligible) & - & 0.10 (negligible)\\ 
\bottomrule
\multirow{2}{*}{\textbf{Category 1: }} & \textbf{Secure mean} 
& 7 & 2 & 14,447 & 9 & 21,419\\ \cline{2-7}
& \textbf{Insecure mean} 
& 18 & 3 & 15,695 & 19 & 37,445\\ \cline{2-7}
\multirow{2}{*}{\textbf{SSL/TLS}}& \textbf{p-value} 
& 0.24 & 3.3e-4 & 0.42 & 0.86 & 0.31\\ \cline{2-7}
& \textbf{Cliff's $\Delta$}
& - & 0.20 (small) & - & - & -\\ 
\bottomrule
\multirow{2}{*}{\textbf{Category 2: }} & \textbf{Secure mean} 
& 5 & 3 & 19,347 & 7 & 16,232\\ \cline{2-7}
& \textbf{Insecure mean} 
& 7 & 3 & 10,057 & 6 & 16,842\\ \cline{2-7}
\multirow{2}{*}{\textbf{Symmetric}}& \textbf{p-value} 
& 0.29 & 0.82 & 0.45 & 0.36 & 0.10\\ \cline{2-7}
& \textbf{Cliff's $\Delta$}
& - & - & - & - & -\\ 
\bottomrule
\multirow{2}{*}{\textbf{Category 3: }} & \textbf{Secure mean} 
& 5 & 2 & 17,079 & 4 & 11,987\\ \cline{2-7}
& \textbf{Insecure mean} 
& 8 & 2 & 14,151 & 3 & 9,470\\ \cline{2-7}
\multirow{2}{*}{\textbf{Asymmetric}}& \textbf{p-value} 
& 0.17 & 0.45 & 0.72 & 0.95 & 0.77\\ \cline{2-7}
& \textbf{Cliff's $\Delta$}
& - & - & - & - & -\\ 
\bottomrule
\multirow{2}{*}{\textbf{Category 4:}} & \textbf{Secure mean} 
& 5 & 2 & 20,382 & 8 & 21,254\\ \cline{2-7}
& \textbf{Insecure mean} 
& 14 & 2 & 20,018 & 22 & 74,482\\ \cline{2-7}
\multirow{2}{*}{\textbf{Hash}}& \textbf{p-value} 
& 0.26 & 0.78 & 0.18 & 0.20 & 0.07\\ \cline{2-7}
& \textbf{Cliff's $\Delta$}
& - & -  & - & - &  -\\ 
\bottomrule
\multirow{2}{*}{\textbf{Category 5:}} & \textbf{Secure mean}
 & 1 & 3 & 33,517 & 0 & 1,031\\ \cline{2-7}
& \textbf{Insecure mean} 
& 21 & 6 & 17,202 & 31 & 56,700\\ \cline{2-7}
\multirow{2}{*}{\textbf{Random}}& \textbf{p-value} 
& 0.04 & 0.02 & 0.27 & 0.02 & 0.01\\ \cline{2-7}
& \textbf{Cliff's $\Delta$}
& 0.58 (large) & 0.68 (large) & - & 0.64 (large) & 0.74 (large)\\ 
\bottomrule
\multicolumn{7}{p{16cm}}{Similar to prior work~\cite{Wang2018}, we interpreted the computed Cliff's delta value $v$ in the following way: 
(1) if $v<0.147$, the effect size is ``negligible''; 
(2) if $0.147\le v<0.33$, the effect size is ``small'; 
(3) if $0.33\le v<0.474$, the effect size is ``medium''; 
(4) otherwise, the effect size is ``large''. 
}\\
\bottomrule
\end{tabular}
\vspace{-1.5em}
\end{table*}

\subsection{Community Dynamics Towards Secure and Insecure Code}
\label{sec:rq2}

For each labeled secure or insecure post, we extracted the following information: (1) score, (2) comment count, (3) the answerer's reputation score, (4) the question's favorite count, and (5) the discussion thread's view count. %We conducted Mann-Whitney U tests to determine whether secure and insecure posts have significant differences for any above-mentioned information types. 



\begin{comment}
\begin{enumerate} 
\item[$I_1$:] score, 
\item[$I_2$:] comment count,
\item[$I_3$:] the answerer's reputation score, 
\item[$I_4$:] the question's favorite count, and
\item[$I_5$:] the discussion thread's view count.
\end{enumerate}
With such information, we checked whether the answerers' reputation scores and other users' activities around the answers manifest different patterns between secure and insecure posts. Specifically, we conducted Mann-Whitney U test~\cite{Fay2010} to determine whether secure and insecure posts have significant differences in terms of any kind of information $I_i (i\in[1, 5])$. We assumed that:

\begin{itemize}
\item[$H_0$:] The number distributions of information $I_i$ between secure and insecure posts are equal; and 
\item[$H_1$:] The number distributions of information $I_i$ between secure and insecure posts are not equal.
\end{itemize}
We chose Mann-Whitney U test to compare two distributions, because the testing method does not require the assumption of normal distributions. 
When $p<0.05$, there is a significant difference between the two groups of posts in terms of $I_i$. In such scenarios, we further computed Cliff's delta~\cite{MACBETH2011} to measure the difference's magnitude. 

\begin{table}
\caption{Comparison between secure and insecure posts}
\label{tab:all}
\scriptsize
\begin{tabular}{C{1.2cm} |rrrr}
\toprule
& \textbf{Secure mean} & \textbf{Insecure mean} & \textbf{p-value} & \textbf{Cliff's $\Delta$}\\
\toprule
\textbf{Score} & \AverScoreSecureAnswers & \AverScoreInsecureAnswers & 0.98 & -\\ \hline
\textbf{Comment count} & \AverCommentsSecureAnswers & \AverCommentsInsecureAnswers & 0.03 & 0.06 (negligible)\\ \hline
\textbf{Reputation} & \AverReputationSecureAnswers & \AverReputationInsecureAnswers &0.02 &0.07 (negligible)\\ \hline
\textbf{Favorite count} & \AverFavoritesSecureAnswers & \AverFavoritesInsecureAnswers & 0.13 & - \\ \hline
\textbf{View count} & \AverViewsSecureAnswers & \AverViewsInsecureAnswers & 0 & 0.09 (negligible)\\
\bottomrule 
\multicolumn{5}{p{8.5cm}}{Similar to prior work~\cite{Wang2018}, we interpreted the computed Cliff's delta value $v$ in the following way: 
(1) if $v<0.147$, the effect size is ``negligible''; 
(2) if $0.147\le v<0.33$, the effect size is ``small'; 
(3) if $0.33\le v<0.474$, the effect size is ``medium''; 
(4) otherwise, the effect size is ``large''. 
}\\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

\textbf{Comparison of Mean Values.}
Table~\ref{tab:all} compares these information categories for the \SecureAnswers\ secure posts and \InsecureAnswers\ insecure ones and applies Mann-Whitney U tests to determine significant results. 
On average, secure posts' answerers have higher  reputation (\AverReputationSecureAnswers\ vs.~\AverReputationInsecureAnswers). However, for the SSL/TLS posts, the insecure answer providers have higher reputation (15,695 vs.~14,447). 
Moreover, insecure posts have higher scores, and more comments, favorites, and views. 
%average values in terms of score, comment count, favorite count, and view count. 
Users seemed to be more attracted by insecure posts,
%, or they found insecure posts more useful. 
\emph{which is counterintuitive}. We would expect secure answers to be seen more favorable; with more votes, comments and views. 

Three reasons can explain our observation. First, software developers often face time constraints. When stuck with coding issues (\emph{e.g.}, runtime errors), developers are tempted to take insecure but simpler solutions~\cite{Meng2018:icse}. %Meng \emph{et al.}~\cite{Meng2018:icse} observed such justifications by SO users for their insecure SSL/TLS usage.
Take the vulnerable SSL/TLS usage in Listing~\ref{lst:ssl} for example. The insecure code was frequently suggested on \SO, and many users voted for it mainly because the code is simple and useful to resolve connection exceptions. 
%Although the code is a simple workaround for runtime errors, 
Nevertheless, the simple solution essentially skips SSL verification and voids the protection mechanism. 
In comparison, a better solution should use certificates from a Certification Authority (CA) or self-signed certificates to drive the customization of \codefont{TrustManager}, and verify certificates with more complicated logic~\cite{certcreate}. 

Second, some insecure algorithms are widely supported by Java-based libraries, which can promote developers' tendency to code insecurely. For instance, up till the current version Java 9, Java platform implementations have been required to support MD5---the well-known broken hash function~\cite{md5java9}. Third, insecure posts are less recent and may have accumulated more positive scores than recent secure posts. 

\begin{tcolorbox}
	\textbf{Finding 3:}
	\emph{On average, insecure posts received higher scores, more comments, more favorites, and more views. 
It implies that (1) more user attention is attracted by insecure answers; and (2) users cannot rely on the voting system to identify secure answers. }
\end{tcolorbox} 

\textbf{Comparison of p-values and Cliff's $\Delta$.}
Table~\ref{tab:all} shows that among all posts, insecure ones obtained significantly more comments ($p=0.02$) and views ($p=1.5\mathrm{e}{-3}$), while the effect sizes are negligible. Specifically for the \emph{Random} category, insecure posts have significantly higher view counts ($p=0.01$) and the effect size is large. 
Meanwhile, 
the owners of secure answer posts have significantly higher reputation ($p=0.02$) but the magnitude is also negligible. 
%(Note that some information including reputation is missing for a few answer writers for reasons that could not be determined.)
%It implies that users with higher reputation are more likely to provide reliable answers. 
%Notice that since some answers' owner information is missing for some reason, we compared reputation scores purely based on the available information of answerers. 

%TODO give percentages
\begin{figure}
\centering
\vspace{-1.1em}
\includegraphics[width=7.5cm]{n-answers-vs-reputation.pdf}
\vspace{-1em}
\caption{The answer distribution based on owners' reputation}
\label{fig:rep}
\vspace{-1.5em}
\end{figure}

Figure~\ref{fig:rep} further clusters answers based on their owners' reputation scores. 
We used logarithmic scales for the horizontal axis, because the scores vary a lot within the range [\LowestReputation, \HighestReputation].
%In Figure~\ref{fig:rep}, the bars between $10^0$ and $10^1$ present the numbers of responders with scores within [1, 10). %Similarly, the bars between $10^1$ and $10^2$ illustrate the number of answers whose providers have scores within [10, 100). 
Overall, 
the secure and insecure answers have similar distributions among different reputation groups. For instance, most answers were provided by users with scores within [$10^2$, $10^4$), accounting for 61\% of secure posts and 68\% of insecure posts.  
% (1) most responders have the lowest reputation (\emph{i.e.}, [0, 5K]); and (2) fewest responders have the highest reputation (\emph{i.e.}, (35K, 40K]).
%Especially, among the 977 users with [0, 5K] scores, 517 people (53\%) provided secure answers. However among the 4 responders with (35K, 40K] scores, 3 people (75\%) offered insecure answers. 
%\SO considers users with at least 20K reputation points as ``trusted users''. In our data set, 
Among the \RelevantAnswersByTrustedUsers\ posts by trusted users, \InsecureAnswersByTrustedUsers\ answers (34\%) are insecure and not reliable. 
One reason to explain why high reputation scores do not guarantee secure answers can be that users earned scores for being an expert in areas other than security. Responders' reputation scores do not necessarily indicate the security property of the provided answers. 
%In such scenarios, high reputation scores do not necessarily have any correlation with the security property of answers suggested by trusted users. 
Therefore, \SO users should not blindly trust the suggestions given by highly reputable contributors.

\begin{tcolorbox}
	\textbf{Finding 4:}
	\emph{The users who provided secure answers have significantly higher reputation than the providers of insecure answers, but the difference in magnitude is negligible. Users cannot rely on the reputation mechanism to identify secure answers. }
\end{tcolorbox} 

\textbf{Comparison of accepted answers. }
It is natural for \SO users to trust accepted answers. 
%and believe that the accepted security-related answers are secure. 
Among the \RelevantAnswers\ posts, we found \AcceptedRelevantAnswers\ accepted answers (38\%). \AcceptedSecureAnswers\ accepted answers are secure, accounting for 38\% of the inspected secure posts. \AcceptedInsecureAnswers\ accepted answers are insecure, accounting for 37\% of the inspected insecure posts. 
It seems that accepted answers evenly distribute among secure and insecure posts; they are not good indicators of suggestions' security property.  
%These numbers imply that users cannot trust accepted answers to identify the secure suggestions. 

\begin{tcolorbox}
	\textbf{Finding 5:}
	\emph{Accepted answers are also not reliable for users to identify secure coding suggestions. }
\end{tcolorbox} 

==> mengsu-icse-2019-4/rq3.tex <==
\subsection{Duplication of Secure and Insecure Code}
\label{sec:rq3}

\begin{figure}
\vspace{-1.1em}
\centering
\includegraphics[width=7.5cm]{group-size-hist.pdf}
\vspace{-1.5em}
\caption{The distribution of clone groups based on their sizes}
\label{fig:size}
\vspace{-1em}
\end{figure}

Among the \RelevantGroups\ security-related clone groups, we explored the degree of code duplication for secure clone groups, insecure groups, and mixed groups. Figure~\ref{fig:size} shows the distribution of clone groups based on their sizes.
Similar to Fig.~\ref{fig:rep}, we used logarithmic scales for both the horizontal and vertical axes. 
In Fig.~\ref{fig:size}, most clone groups are small, with 2-3 similar snippets. The number of groups decreases 
%with the group size. 
dramatically as the group size increases. 
Interestingly, within $[2^4, 2^6)$, there are more insecure groups than secure ones.
Table~\ref{tab:size} compares the sizes of secure and insecure groups. 
%We used the Mann-Whitney U test to compare the sizes of secure and insecure groups (see Table~\ref{tab:size}). 
Surprisingly, insecure groups have significantly larger sizes than secure ones, although the difference is negligible. 
Our observations imply that \emph{the frequently mentioned code snippets on \SO are not necessarily more secure than less frequent ones}. Users cannot trust code's repetitiveness to decide the security property. 
%or the horizontal axis, because the number of clone instances in each group varies a lot. The largest clone group contains 65 instances, 
%which securely generate release key hashes for an app to communicate with Facebook, as shown in Figure~\ref{fig:}
%while each of the smallest groups has 2 instances. In Figure~\ref{fig:size}, 
%The bars between $2^1$ and $2^2$ present the number of groups that contain 2 or 3 instances. 
%Similarly, the bars between $2^2$ and $2^3$ illustrate the number of groups with 4, 5, 6, or 7 instances. 
%We also used logarithmic scales for the vertical axis, because the number of groups within each size range also varies a lot. 
%For instance, within $[2^1, 2^2)$, there are 759 groups, including 479 secure groups, 251 insecure groups, and 29 mixed groups. Nevertheless, within the range $[2^6, 2^7)$, there is only one secure group. 

\begin{table}
\caption{Comparison between secure and insecure groups in terms of their group sizes}
\label{tab:size}
\vspace{-0.5em}
\scriptsize
\begin{tabular}{c| R{1.7cm} R{1.7cm} R{1.2cm} R{1.7cm}}
\toprule
& \textbf{Secure groups' mean} & \textbf{Insecure groups' mean} & \textbf{p-value} & \textbf{Cliff's $\Delta$}\\ 
\toprule
\textbf{Size} & \SecureGroupMeanSize & \InsecureGroupMeanSize & \GroupSizePValue & \GroupSizeCliff\ (negligible)\\
\bottomrule
\end{tabular}
\vspace{-1.5em}
\end{table}

\begin{tcolorbox}
	\textbf{Finding 6: }
	\emph{
	Repetitiveness does not guarantee security, 
	 %guarantee security correctness. 
	%The repetitively suggested code snippets are not necessarily secure, 
	so users cannot assume 
	a snippet to be secure simply because it is recommended many times. 
	}
\end{tcolorbox} 

To understand why there are mixed groups that contain similar secure and insecure implementations, we conducted a case study on  10 randomly selected mixed groups. Among \textit{all} these groups, secure snippets differ from insecure ones by using distinct parameters when calling security APIs.
This implies a great opportunity to build security bug detection tools that check for the parameter values of specific APIs. 

\begin{lstlisting}[caption=A clone group with both secure and insecure code, label=lst:clones]
(*\bfseries // An insecure snippet using AES/ECB to create a cipher~\cite{clone1}*)
Cipher cipher = Cipher.getInstance("AES/ECB/PKCS5Padding", "SunJCE");
Key skeySpec=KeyGenerator.getInstance("AES").generateKey();
cipher.init(Cipher.ENCRYPT_MODE, skeySpec);
System.out.println(Arrays.toString(cipher.doFinal(new byte[] { 0, 1, 2, 3 })));
(*\bfseries //A secure snippet using AES/CFB to create a cipher~\cite{clone2}*)
final Cipher cipher=Cipher.getInstance("AES/CFB/NoPadding", "SunJCE");
final SecretKey skeySpec=KeyGenerator.getInstance("AES").generateKey();
cipher.init(Cipher.ENCRYPT_MODE, skeySpec);
System.out.println(Arrays.toString(cipher.doFinal(new byte[] { 0, 1, 2, 3 })));
\end{lstlisting}

Listing~\ref{lst:clones} shows a mixed clone group, where the insecure code uses ``\codefont{AES/ECB}'' to create a cipher, and the secure code uses ``\codefont{AES/CFB}''. 
%passes a different parameter for cipher creation. 
Actually, both snippets were provided by the same user, which explains why they are so similar. These answers are different because the askers inquired for different modes (ECB vs.~CFB). Although the answerer is an expert in using both APIs and has a high reputation score 27.7K, he/she did not mention anything about the vulnerability of ECB. This may imply a lack of security expertise or vulnerability awareness of highly reputable \SO users, and a well-motivated need for automatic tools to detect and fix insecure code.  

\begin{tcolorbox}
	\textbf{Finding 7: }
	\emph{
	Secure and insecure code in the same mixed group often differs 
	by passing distinct parameters to the same security APIs highlighting opportunities for automatic tools to handle security weaknesses. 
	}
\end{tcolorbox} 


==> mengsu-icse-2019-4/rq4.tex <==
\subsection{Creation of Duplicated Secure and Insecure Code}
\label{sec:rq4}

We conducted two case studies to explore
why duplicated code was suggested.  

%there are duplicated code suggested on \so.

\textbf{Case Study I: Duplicated answers by different users.} 
We examined the largest secure group and largest insecure group. 
The secure group has 65 clone instances, which are similar to the code in Listing~\ref{lst:facebook}. 
These snippets were offered to answer questions on how to enable an Android app to log into Facebook. 
The questions are similar but different in terms of the askers' software environments (\emph{e.g.}, libraries and tools used) and potential solutions they tried. Among the 65 answers, only 18 (28\%) were marked as accepted answers. %It implies that
The majority of duplicated suggestions are relevant to the questions, but cannot solve the issues. 
\SO users seemed to repetitively provide ``generally best practices'',  
%advice even though the advice is not helpful;
probably because they wanted to earn points by answering more questions. 
%although they are not sure whether the suggestions are helpful. %This may be because users wanted to earn points by answering more questions. 
%provide relevant answers even though they are not quite sure whether the answers can be helpful. Therefore, it is possible that SO developers can build mappings between questions and answers, and automatically recommend related answers to a given question. Although such solutions do not necessarily always lead to accepted answers, at least it can save developers' effort and time of posting and checking redundant but useless suggestions. 

\begin{lstlisting}[caption=An exemplar snippet to generate a key hash for Facebook login~\cite{facebook}, label=lst:facebook]
PackageInfo info = getPackageManager().getPackageInfo("com.facebook.samples.hellofacebook", PackageManager.GET_SIGNATURES);
for (Signature signature : info.signatures) {
  MessageDigest md = MessageDigest.getInstance("SHA");
  md.update(signature.toByteArray());
  Log.d("KeyHash:", Base64.encodeToString(md.digest(), Base64.DEFAULT)); }
\end{lstlisting}

The largest insecure group contains 32 clone instances, which are similar to the code 
in Listing~\ref{lst:ssl}. The questions are all about how to implement SSL/TLS or resolve SSL connection exceptions. 13 of these answers (41\%) were accepted. We noticed that only one answer warns ``\emph{Do not implement this in production code \ldots}''~\cite{sslwarn}.
Six answers have at least one comment talking about the vulnerability.  
The remaining 25 answers include nothing to indicate the security issue.  
%mention nothing about the security property. 

\textbf{Case Study II. Duplicated answers by the same users.} %We examined the duplicated answers provided by the same users. 
In total, \AnswerReusageUsers\ users reused code snippets to answer multiple questions. 
Among the \RelevantGroupsOfReusedAnswers\ clone groups these users produced, there are \SecureGroupsOfReusedAnswers\ secure groups, \InsecureGroupsOfReusedAnswers\ insecure groups, and 
\MixedGroupsOfReusedAnswers\ mixed groups. 
\SecureReusageUsers\ users repetitively posted secure answers, and \InsecureReusageUsers\ users posted duplicated insecure answers. Six among these users posted both secure and insecure answers. 
%\todo{X} of the 109 users posted two duplicated answers (\emph{i.e.}, clone pairs) in our data set. \todo{...}
Most users (\emph{i.e.}, 92) only copied code once and produced two duplicates. One user posted nine insecure snippets, with seven snippets using an insecure version of TLS, and two snippets trusting all certificates. 
This user has 17.7K reputation (top 2\% overall) and is an expert in Android. By examining the user's profile, we did not find any evidence to show that the user intentionally misled people. It seems that the user was not aware of the vulnerability when posting these snippets.

To understand whether duplicated code helps answer questions, we randomly sampled 103 (of the 208) clone groups resulting in \SecureSamplePairs\ secure clone pairs, \InsecureSamplePairs\ insecure pairs, and \MixedSamplePairs\ mixed pairs. 
%We inspected these snippets to check whether they actually helped answer the questions.
Unexpectedly, we found that \ReusedPairsForDiffQ\ pairs (45\%) did not directly answer the questions. 
For instance, a user posted code without reading the question and received down-vote (i.e., $-1$)~\cite{noread}.
%A user posted an answer to advertise the library he wrote~\cite{advertise} or posted code without reading the question~\cite{noread}. %For example, an answer obtained ``-1'' score and the comment said: ``\emph{Obligatory down-vote because you simply posted the exact same code again. ... If you're going to post code, at least edit it to match the constraints as established in the question}''~\cite{noread}.  
In the other 57 cases, duplicated code was provided to answer similar or identical questions.
% although essentially responders can avoid such duplication by offering the URL links to their single-copy original answers. 
%A comment helps explain the reason for duplication: ``\emph{Posting links as answer are not recommended as these answer becomes obsolete if link goes down/dead. I would suggest you to add how you solved in elaborated form. So that any user who gets to this page will get everything in this page only. Plus you will get up-votes too for writing good answer}''~\cite{explainclone}. Thus, answerers are motivated to copy and paste code to provide better posts and earn more reputation. 

%(2) responders provided high-quality self-contained similar answers; and 
\begin{tcolorbox}
	\textbf{Finding 8: }
	\emph{Duplicated answers were created because (1) users asked  similar or related questions; and (2) some users blindly copied and pasted code to answer more questions and earn points. 
	However, we did not identify any user that intentionally misled people by posting insecure answers. 
	}
\end{tcolorbox} 


==> mengsu-icse-2019-4/suggestion.tex <==
\section{Our Recommendations}
\label{sec:suggestion}

By analyzing \SO answer posts relevant to Java-based security library usage, we observed the wide-spread existence of insecure code. 
It is worrisome to learn that \SO users cannot rely on either the  reputation mechanism or voting system to infer
an answer's security property, 
%whether a security-relevant \SO answer is secure or not, 
%mainly because the answerers are also unaware of the security property or they do not care about that. 
A recent Meta Exchange discussion thread also shows the frustration of \SO developers to keep outdated security answers up to date~\cite{metaexchange}. Below are our recommendations based on this analysis. 

\paragraph{\textbf{For Tool Builders}} Explore approaches that accurately and flexibly detect and fix security bugs. 
Although a few tools identify security API misuses through static program analysis or machine learning~\cite{Egele:2013,He2015,Rahaman:2017,fischer:2017}, they are unsatisfactory due to the (1) hard-to-extend API misuse patterns hardcoded in tools, and (2) hard-to-explain machine learning results.
People report vulnerabilities and patches on CVE and in security papers. Tools like LASE~\cite{Meng2013:Lase} were built to (i) generalize program transformation from concrete code changes, and (ii) leverage the transformation to locate code for similar edits. If tool developers can extend such tools to compare secure-insecure counterparts, they can automatically fix vulnerabilities in a flexible way. 

%We suggest developing new approaches that (i) compare identified insecure implementations with secure counterparts,  (ii) generalize bug patterns and fixing strategies from the comparison, and (iii) search for buggy code matching any pattern to suggest security fixes. 

\paragraph{\textbf{For \SO Developers}} Integrate static checkers to scan existing corpus and \SO posts under submission. Automatically add warning messages or special tags to any post that has vulnerable code. Encourage moderators or trusted users to exploit clone detection technologies in order to efficiently detect and remove both duplicated questions and answers. Such deduplication practices will not only save users' time and effort of reading/answering useless duplicates, but also mitigate the misleading consensus among multiple similar insecure suggestions. 
As user profiles include top tags to reflect the frequently asked/answered questions by users. instead of accumulating a single reputation score for each user, SO developers can compute one score for each top tag to better characterize users' expertise. 

%Instead of presenting a responder's overall reputation score to indicate an answer's credibility, show the responder's score in related areas or for the specific tags.

\paragraph{\textbf{For Designers of Crowdsourcing Platforms}}
%Recruit a volunteer code auditing team that check some of the most popular security-related posts periodically (\emph{e.g.}, once every week) to identify and report security issues. 
Provide incentives to users for downvoting or detailing vulnerabilities and suggesting secure alternatives. 
Introduce certain mechanisms to encourage owners of outdated or insecure answers to proactively archive or close such posts. 
%Currently on \so, a user loses reputation for downvoting posts. 
%if a user downvotes a post, the user loses two reputation points~\cite{so-priviledges}. 
%In the future,  platforms can instead encourage security experts to downvote insecure answers by rewarding them with reputation points. 
We expect researchers from the usable security and HCI domain to evaluate and test new design patterns that integrate security evaluation in the gamification approach.

%The current incentive systems seem to encourage users to repetitively post compilable or executable quickfix solutions, regardless the security property of any solution. 



%\paragraph{\textbf{For \SO Users}} Be cautious when taking security-related suggestions on \SO. Do not blindly trust an answer's acceptance status, vote, favorite count, responder's reputation, view count, comment, or timestamp to infer whether an answer is secure or not. 
%Pay attention to the security property when using security APIs, instead of purely focusing on code's compilability or executability. Refer to more reliable information resources, such as API official documentation and books, for security awareness education purposes. Responsibly post security-related answers, and warn about the vulnerabilities if insecure solutions are necessary. 

==> mengsu-icse-2019-4/threats.tex <==
\section{Threats to Validity}
\label{sec:threats}

\paragraph{Threat to External Validity}
This study labels insecure code based on the Java security rules summarized by prior work~\cite{fischer:2017}, so our studied insecure snippets are limited to Java code and these rules. Since we used the state-of-the-art insecurity criteria, our analysis revealed as diverse insecure code as possible. In the future, we plan to identify more kinds of insecure code by considering different programming languages and exploiting multiple vulnerability detection tools~\cite{flawFinder,checkmarx}.

%more security rules, and more scalable labeling techniques. 

\paragraph{Threat to Construct Validity}
Although we tried our best to accurately label code, our analysis may be still subject to human bias and cannot scale to handle all crawled data or more security categories. We conservatively assume a snippet to be secure if it does not match any given rule. However, it is possible that some labeled secure snippets actually match the insecurity criteria not covered by this study, or will turn out to be insecure when future attack technologies are created. 
We concluded that insecure answers are popular on \SO and gain high scores, votes, and views. 
Even if the labels of some existing secure answers will be corrected as insecure in the future, our conclusion generally holds. 
%, despite potential changes in detailed results, it will only strengthen our general conclusion: insecure answers are popular and may mislead developers. 
%In the future, we will develop extensible approaches that accurately label code snippets. 

\paragraph{Threat to Internal Validity}
We leveraged clone detection to sample the extracted code snippets and reduce our manual analysis workload. Based on code's occurrence repetition, clone detection can ensure the representativeness of sampled data. However, the measurement on 
a sample data set may be still different from that of the whole data set. Once we build automatic approaches to precisely identify security API misuses, we can resolve this threat. 


==> rebuttal.tex <==
We thank all reviewers for the insightful comments. We will remove the statement about SO users intentionally submitting insecure answers, and add a discussion on existing vulnerability detection tools.

A. R1: How we use Baker. 

We included a code snippet if Baker finds at least one API (class or method) with an exact match. However, Baker's result-set is not fully precise and requires a number of post-processing steps to reduce false positives. These include a blacklist filter for standard Java types and very popular methods, e.g. equal(), put(), get(), read(), write(). Bakers oracle contains only the given security APIs, which helped reduce false positives (case 1) but did not help reduce false negatives (case 2).

B. R1&3: Selection of snippets. 

By detecting clones among the 25,855 snippets, we identified 2,657 clone groups (with at least two snippets in each group) that in total contain 8,690 snippets. We manually inspected each of the 8,690 snippets, identifying 1,784 secure snippets, 1,337 insecure ones, and 5,569 irrelevant ones (Table III). When mapping labeled snippets to their owner posts, we consider a post insecure if it contains any labeled insecure code. A post was labeled secure if it did not contain an insecure snippet and at least one secure snippet.

C. R2 questions novelty. 

Our work investigates the evolution and distribution of secure and insecure coding suggestions within the SO ecosystem itself, while [5] investigates their migration to real-world apps. 

While [5] compares average score and view counts for secure and insecure snippets, they merely do this for snippets whose exact copies have migrated into apps but not for our much broader set of snippets on SO. Therefore, the dataset of [5] is not representative to evaluate the impact of severity, community's awareness, and popularity of unreliable SO suggestions on secure coding. 

We conducted not only statistical testing on a comprehensive dataset to quantitatively contrast score, view count, comment count, reputation, and favorite count, but also performed case studies to qualitatively analyze the differences. We further explored the missing link between gamification and security advice quality on crowdsourcing platforms. 

D. R2 asks for concrete suggestions.

i) For tool builders: People report vulnerabilities and patches on CVE and in security papers. Tools like LASE (ICSE13) were built to (1) generalize program transformation from concrete code changes, and (2) leverage the transformation to locate code for similar edits. If tool developers can extend such tools to compare secure-insecure counterparts, they can automatically fix vulnerabilities. 

ii) For SO developers: User profiles include top tags, which reflect the frequently asked/answered questions by users. Instead of accumulating a single reputation score for each user, SO developers can compute one score for each top tag to better characterize users' expertise. 

iii) For crowdsourcing designers: We expect researchers from the usable security and HCI domain to evaluate and test new design patterns that integrate security evaluation in the gamification approach.

E. R2 questions verifiability.
We support open science and will therefore open source our complete labeled data set and tools.




